Component Stability in Low-Space Massively Parallel Computation

We study the power and limitations of component-stable algorithms in the low-space model of Massively Parallel Computation (MPC). Recently Ghaffari, Kuhn and Uitto (FOCS 2019) introduced the class of component-stable low-space MPC algorithms, which are, informally, defined as algorithms for which the outputs reported by the nodes in different connected components are required to be independent. This very natural notion was introduced to capture most (if not all) of the known efficient MPC algorithms to date, and it was the first general class of MPC algorithms for which one can show non-trivial conditional lower bounds. In this paper we enhance the framework of component-stable algorithms and investigate its effect on the complexity of randomized and deterministic low-space MPC. Our key contributions include: 1) We revise and formalize the lifting approach of Ghaffari, Kuhn and Uitto. This requires a very delicate amendment of the notion of component stability, which allows us to fill in gaps in the earlier arguments. 2) We also extend the framework to obtain conditional lower bounds for deterministic algorithms and fine-grained lower bounds that depend on the maximum degree $\Delta$. 3) We demonstrate a collection of natural graph problems for which non-component-stable algorithms break the conditional lower bound obtained for component-stable algorithms. This implies that, for both deterministic and randomized algorithms, component-stable algorithms are conditionally weaker than the non-component-stable ones. Altogether our results imply that component-stability might limit the computational power of the low-space MPC model, at least in certain contexts, paving the way for improved upper bounds that escape the conditional lower bound setting of Ghaffari, Kuhn, and Uitto.

==> ComponentInstability.tex <==





\renewcommand{\spac}{\ensuremath{\mathfrak{s}}\xspace}




\section{Definitions}

\begin{definition}
	An \textbf{input family} $\mathcal G$ is a hereditary class of graphs in which for any graph $H\in \mathcal G$, all nodes possess IDs such that any two nodes in the same connected component have different IDs.
	
	We will use the notation $H\in_{n,\Delta} \mathcal G$ to mean that $H\in \mathcal G$, and $H$ has at most $n$ nodes and maximum degree at most $\Delta$.
\end{definition}

We define the LOCAL lower bounds we will consider:
\begin{definition}
	Let $\mathcal G$ be an input family. Given a graph problem $P$, a function $T:\nat\rightarrow\nat$ is a \textbf{uniform deterministic LOCAL lower bound on $\mathcal G$ ($\mathcal G$-UDLB)} for $P$  if no deterministic LOCAL algorithm can solve $P$ in $T(n,\Delta)$ rounds on all graphs $G \in_{n,\Delta}\mathcal G$ with at most $n$ nodes and with maximum degree at most $\Delta$, even if all nodes are provided with the value $T(n,\Delta)$.
\end{definition}
Note that we do not provide nodes with a function of the \emph{actual} number of nodes and maximum degree of the network, and only require that these are \emph{at most} $n$ and $\Delta$ respectively. This is in order to include lower bounds which do not hold if nodes know these exact values.

\begin{definition}
	A $(\alpha,\beta)$-MPC algorithm for a problem $P$ on $\mathcal G$ is a deterministic algorithm which solves $P$ on all inputs $H\in_{n,\Delta}\mathcal G$ using $O(n^\alpha)$ local space and $O(n^\beta + n\Delta)$ global space.
\end{definition}

We need not specify what information about number of nodes and maximum degree MPC algorithms are given in advance, since they can compute those values exactly in $O(1)$ rounds with low-space.
\begin{lemma}
	If there exists an $(\alpha,\beta)$-MPC algorithm $A_{MPC}$ which solves a problem $P$ on graphs $H\in_{n,\Delta}\mathcal G$ in $T(n,\Delta)$ rounds, then there exists an $(\alpha,\beta)$-MPC algorithm $A'_{MPC}$ which solves $P$ on graphs $H\in_{n,\Delta}\mathcal G$ in $T(n,\Delta)+O(1)$ rounds, with the additional property that its output is independent of the initial assignment of input to machines.
\end{lemma}

\begin{proof}
	By \cite{GSZ11}, there exists an $O(1)$-round algorithm for sorting on low-space MPC (i.e. for any constant $\alpha>0$). Therefore, in $O(1)$ rounds we can re-organize the entire input into a fixed canonical assignment to machines. So, we can construct the algorithm $A'_{MPC}$ by simply sorting the input in this way, and then simulating $A_{MPC}$.
\end{proof}

The implication of this observation is that we now need only consider MPC algorithms with this assignment-independence property, since any asymptotic lower bound against such algorithms necessarily holds for all algorithms. Henceforth, therefore, we need not specify the initial assignment of input to machines when running MPC algorithms, since we can assume it has no effect on output.	

\section{Deterministic MPC Conditional Lower Bounds}


We now show a deterministic analog of the lower-bounds framework of \cite{GKU19}. In some ways determinism makes the argument simpler since we need not keep track of success probabilities of algorithms. However, \cite{GKU19} uses some randomized algorithms within their reductions, which we must take care to derandomize. We also make some generalizations in order to expand the range of lower bounds to which the results apply:

\begin{itemize}
	\item We keep track of dependency on maximum degree $\Delta$ in order to incorporate lower bounds with such dependency;
	\item We clarify the assumptions made on knowledge of $n$ and $\Delta$ in LOCAL algorithms, in order to include lower bounds which do not hold under exact knowledge;
	\item We extend to bounds applying to any hereditary class of graphs, rather than only to the class of all graphs. This allows us to consider comparable upper bounds for problems which are not possible on all graphs, such as $\Delta$-coloring.
\end{itemize}

\begin{lemma}\label{lem:centergraphs}
Let $P$ be a graph problem for which there is a $T(n,\Delta)$-round $\mathcal G$-UDLB. Then, for every $(\alpha,\beta)$-MPC algorithm $A_{MPC}$ that solves $P$ on $\mathcal G$, there are two $T(n,\Delta)$-hop-indistinguishable centered graphs $G,G'\in_{n,\Delta} \mathcal G$, such that $A_{MPC}$ gives different outputs at their center.
\end{lemma}

\begin{proof}
	We construct a LOCAL algorithm $A_{LOCAL}$ to run on graphs $H\in_{n,\Delta} \mathcal G$ as follows: each node $v \in H$ collects its $T(n,\Delta)$-hop neighborhood (recall that we can assume all nodes are provided with the value $T(n,\Delta)$), simulates $A_{MPC}$ on this graph, and outputs $A_{MPC}(v)$.
	
	If $A_{MPC}$ gives the same output for every two $T(n,\Delta)$-hop-indistinguishable centered graphs $G,G'\in_{n,\Delta} \mathcal G$, then it gives the same result for the center node $v$ of each simulated ball $B_{T(n,\Delta)}(v)$ as it would when run on $H$ as a whole. This follows since each $B_{T(n,\Delta)}(v)$ is indeed $T(n,\Delta)$-hop-indistinguishable from the same ball in $H\in_{n,\Delta} \mathcal G$, and since $\mathcal G$ is a hereditary class of graphs, we also have $B_{T(n,\Delta)}(v)\in_{n,\Delta} \mathcal G$. $A_{MPC}$ gives a valid output on $H$, and therefore $A_{LOCAL}$ also gives a valid output, contradicting the assumed lower bound. So, there must be two $T(n,\Delta)$-hop-indistinguishable centered graphs $G,G'\in_{n,\Delta} \mathcal G$ such that $A_{MPC}$ gives different outputs at their center.
\end{proof}

\begin{lemma}\label{lem:lb4.2}
	Let $P$ be a graph problem with a $D:=T(n,\Delta)$-round $\mathcal G$-UDLB, where $D=o(\frac{\log n}{\log\log n})$. Suppose that there is an $o(\log D)$-round component-stable $(\alpha,\beta)$-MPC algorithm $A_{MPC}$ that solves P on all graphs $G\in_{n,\Delta} \mathcal G$, for $\alpha\in(0,1)$ and $\beta>0$. Then, we obtain a $(2\alpha,(1+\alpha)(1+\beta))$-MPC algorithm $B_{st-conn}$ with round complexity $o(\log T(n^{1+\alpha/2},\Delta))$ for $D$-diameter s-t connectivity.
\end{lemma}

\begin{proof}
	By \cref{lem:centergraphs} (using $n^{\alpha/2}$ in place of $n$), we have two $T(n^{\alpha/2},\Delta)$-hop-indistinguishable centered graphs $G,G'\in_{n^{\alpha/2},\Delta} \mathcal G$, such that $A_{MPC}$ gives different outputs at their center $v$.
	
	We now construct an $(\eps,\beta)$-MPC algorithm for $D$-diameter s-t connectivity, which will work by combining the results of several parallel simulations. We run a parallel simulation for each function $h$ in a $(D^{-2D},D)$-wise independent family $\mathcal{H}$ as given in \cref{cor:hashschedule}. There are, therefore, $n^{o(1)}$ parallel simulations. Given an $n$-node input graph $H$ for $D$-diameter s-t connectivity, with special nodes designated $s$ and $t$, and for each $h\in \mathcal{H}$, we do the following:
	
	We first discard all nodes of degree higher than $2$. Then, for each remaining node in $H$ we collect its $1$-hop neighborhood onto a machine (this takes $O(1)$ rounds and does not increase asymptotic space usage). Each node of $H$ then drops out if its $1$-hop neighborhood is not consistent with being part of an $s-t$ path with consecutively increasing values under $h$ (other than the value of $h(t)$, which we make no requirements for). In particular:
	
	\begin{itemize}
		\item Nodes $s$ and $t$ in $H$ must have degree $1$ (and otherwise we terminate the simulation immediately and output \NO).
		\item Other nodes must have degree $2$, and the values of $h$ in their $1$-hop neighborhood must be a consecutive triplet (other than $h(t)$).
	\end{itemize}
	
	Every remaining node (i.e., satisfying these conditions) in $H$ is assigned (copies of) nodes in $G$ and $G'$ as follows:
	
	\begin{itemize}
		\item Node $s$ in $H$ is assigned all nodes of distance at most $h(s)$ from $v$ in $G$ and $G'$.
		\item Node $t$ in $H$ is assigned all nodes of distance more than $D$ from $v$ in $G$ and $G'$.
		\item Other nodes $u$ in $H$ are assigned the nodes of distance exactly $h(u)$ from $v$ in $G$ and $G'$.
	\end{itemize}
	
	We then construct new graphs $G_H$ and $G'_H$ as follows:
	
	The vertex sets of $G_H$ and $G'_H$ consist of every assigned copy of nodes in $G$ and $G'$ respectively.
	
	Let $w_{u}$ in $G_H$ denote a copy of $w$ in $G$, assigned to vertex $u$ in $H$. We place an edge between $w_{u}$ and $\hat w_{\hat u}$ in $G_H$ iff $w\sim_G \hat w$ and $u\sim_H \hat u$ (or $u=\hat u$). This graph can easily be constructed in $O(1)$ rounds of MPC, using $O(n^{\alpha})$ local space and $O(n)$ global space, since machines each need only store $G$, $G'$, and $O(n^{\alpha})$ edges of $H$. We construct $G'_H$ from $G'$ analogously. We set $ID(w_{u}) = ID(w)$, i.e., we keep identifiers identical to the simulated node in $G$ or $G'$, and do not encode the simulating node in $H$. This means that identifiers in $G_H$ and $G'_H$ are not necessarily unique, but we can see that they are unique within connected components, since no two copies of the same node in $G$ or $G'$ can be connected in $G_H$ or $G'_H$.
	
	We also see that the connected components of $G_H$ and $G'_H$ are identical to induced subgraphs on $G$ and $G'$ respectively. In particular, we consider the topology of the connected components $CC({v_{s}})$ and $CC'(v_{s})$ containing $v_{s}$ in $G_H$ and $G'_H$ respectively:
	
	\begin{enumerate}
		\item If $s$ and $t$ are endpoints of a path of $p\le D+1$ \emph{nodes} (and therefore of \emph{length} at most $D$) in $H$, $h(s)=p-D$, and $h(u_i) = p-D+i$ for each $u_i\ne t$ which is the node at distance $i$ along the path from $s$, then $CC({v_{s}}) =  G$ and $CC'(v_{s}) = G'$;
		\item otherwise, $CC(v_{s})=CC'(v_{s})$.
	\end{enumerate}
	
	In the first case, this is because the nodes on the $s-t$ path are together assigned precisely one copy of each on the nodes in $G$ and $G'$, in such away that every two adjacent nodes in $G$ and $G'$ are assigned to adjacent nodes on this path. In the second case, the only nodes that differ in $G$ and $G'$ are assigned only to $t$, and no outputs of $h$ can cause these to be connected to $v_{s}$. Therefore the graphs of nodes that \emph{are} connected to $v_{s}$ are identical.
	
	We now simulate $A_{MPC}$ on $G_H$ and $G'_H$. The output for each of the concurrent simulations is \YES if $A_{MPC}(v_{s})$ differs on $G_H$ and $G'_H$, and \NO otherwise, and the \emph{overall} output is \YES iff any of the simulation outputs was \YES.
	
	If $s$ and $t$ are endpoints of a path of length at most $D$ in $H$, then by \cref{cor:hashschedule} there is some $h\in\mathcal H$ in which all nodes on the path have the `correct' output from $h$ (i.e., as specified in point $1$ above). During the simulation with this $h$, we then have $CC({v_{s}}) =  G$ and $CC'(v_{s}) = G'$. Since $A_{MPC}$ is component-stable, its output for $v_{s}$ in both cases is equal to its output on $v$ in $G$ and $G'$ respectively, and by our choice of $G$ and $G'$, these are different. Therefore, the simulation output, and the overall output, is correctly \YES.
	
	If $s$ and $t$ are not endpoints of a path of length at most $D$ in $H$, then in all simulations we have $CC({v_{s}})=CC'({v_{s}})$. Since $A_{MPC}$ is component-stable, its output depends (deterministically) on these connected components, and is therefore the same in both cases. Final output is then correctly \NO.
	
	In both cases, we have $G_H$ and $G'_H\in_{n^{1+\alpha/2},\Delta} \mathcal G$, since:
	
	\begin{itemize}
		\item The number of nodes in $G_H$ and $G'_H$ is at most the number of vertices in $H$ multiplied by the number in $G$ and $G'$, i.e. at most $n^{1+\alpha/2}$
		\item The maximum degree in $G_H$ and $G'_H$ is at most $\Delta(n^{\alpha/2}) \le \Delta(n^{1+\alpha/2})$, and the number of edges is at most $N^{1+\alpha}$ (because each node in $H$ contributes at most $|E(G)|$ and $|E(G')|\le n^{\alpha}$ edges)
		{\color{red}  \item Node IDs are unique within their connected component - but not in the whole graph, so this is not a valid input under standard definitions of MPC algorithms
}	\end{itemize}
	
	$A_{MPC}$ therefore runs correctly on $G_H$ and $G'_H$ in $o(\log T(n^{1+\alpha/2},\Delta))$ rounds.
	\footnote{\cite{GKU19} effectively uses $T(n^{1+\alpha/2},\Delta) = poly(T(n,\Delta))$ to simplify here, which is true for most reasonable functions $T$ but not technically true in general. $T(n,\Delta)= f(\lfloor f^{-1}( n)\rfloor)$, for some very fast-growing function $f$ (e.g. triple exponential) is a counterexample.}
	We run $O(n^{o(1)})$ concurrent simulations, each of an $(\alpha,\beta)$-MPC algorithm running on an input of size $n^{1+\alpha/2}$, i.e., requiring $O(n^{\alpha+\alpha^2/2})$ local and $O(n^{\beta+\alpha\beta/2}+n^{1+\alpha})$ global space. The total space requirements are therefore at most $O(n^{2\alpha})$ local space and $O(n^{(1+\alpha)(1+\beta)})$ respectively.
\end{proof}

\begin{lemma}\label{lem:1v2cycle}
Suppose that every $(\alpha,2+\beta+o(1))$-MPC algorithm that can distinguish one $n$-node cycle from two $n/2$-node cycles requires $\Omega(\log n)$ rounds. Then, any $(\alpha,\beta)$-MPC algorithm that solves $D$-diameter s-t connectivity for $D =o(\frac{\log n}{\log\log n})$ requires $\Omega(\log D)$ rounds.

\end{lemma}

\begin{proof}
Suppose for the sake of contradiction that we have an $(\alpha,\beta)$-MPC algorithm $A$ that solves $D$-diameter s-t connectivity in $o(\log D)$ rounds. We proceed similarly to Lemma 4.1 of \cite{GKU19} to construct an $(\alpha,2+\beta+o(1))$-MPC algorithm $B$ for distinguishing one-vs-two cycles, replacing random choices with derandomized versions.

The first step is to build an algorithm $A'$ for the following connected component identification problem: given a graph $H$ with unique node IDs, all nodes should be given labels such that any connected component which is a path of length at most $D$ has the same label for each node, and any two nodes of different components receive different labels.

We will run $O(n^2)$ parallel instances of $A$. We divide the instances into at most $n$ groups, where in each group we set the designated sink node $t$ to be one of the nodes of degree $1$ in the input graph $H$. Then, in each group, we have $O(n)$ tests, one for each choice of $s$ as a node of degree $1$ or $2$ in $H$, and in the case $deg(s)=2$, we further divide into two cases where $s$ discards either one of its two adjacent edges. In this way, for any path of length at most $D$, there will be a instance on which $A$ is run with this path as a connected component and $s$ and $t$ as the endpoints, and will return \YES.

The output for a node $v\in H$ under $A'$ will be the minimum ID of node $w$ such that a instance of $A$ returned \YES with $s = v$ and $t=w$ (if there are no such instances, it returns its own ID). Any two nodes on connected component which is a path of length at most $D$ therefore have the same output: the minimum ID of a node on that path. Any two nodes in different components are given different labels, which are IDs of nodes in their connected component. So, we have an algorithm for the component identification problem as stated.

The next step is to use $A'$ to build an algorithm $B$ for the one-vs-two cycle problem, on an input $2$-regular graph $G$. We have $O(\log_D n)$ sequential iterations, each of which works as follows:

We run $n^{o(1)}$ parallel instances, each using one of the functions $h$ from a $(D^{-2D},D)$-wise independent family $\mathcal{H}$ (as given in \cref{cor:hashschedule} and used in proof of \cref{lem:lb4.2}). We use this function $h$ to map edges to $[\sqrt{(D)}]$, and remove from the graph all edges $e$ with $h(e)=1$ (i.e. we are effectively derandomizing the process of removing each edge with probability $D^{-1/2}$ as done in \cite{GKU19}).

We then run $A'$ on the resulting graph, giving each node a label. We can collect all nodes of the same label (and their adjacent edges, including those with $h(e)=1$) onto a machine, in $O(1)$ rounds. This machine then contracts all such nodes which form a connected component which is a path (or cycle) of length at most $D$ into a single node, giving this new supernode the ID of any of its component nodes, and updating all adjacent edges (which are all held by the machine) accordingly.

Machines then count the number of edges they contracted, and we sum these values for each of the parallel instances (i.e. under each hash function $h$) in $O(1)$ rounds. The instance in which most total edges were contracted is chosen, and we proceed to the next sequential iteration on the graph resulting from that instance.

We analyze the number of sequential iterations needed. Under a random choice of $h\in \mathcal H$, on a graph with $m$ edges, we can bound the number of contracted edges as follows: each edge $e$ has probability at most $2 D^{-1/2}$ of not falling in a component which is a path (or cycle) of length at most $D$ after edges $e'$ with $h(e')=1$ are removed. This is because $e$ has probability at most $D^{-1/2}+D^{-2D}$ of being removed itself, and the probability that at least $\frac D2$ edges along the path in one direction from $e$ all remain is at most $2(1-D^{-1/2})^\frac D2 + 2D^{-2D}\le \frac 12 D^{-1/2}$. If $e$ does fall in a component which is a path (or cycle) of length at most $D$, it will be contracted. Therefore, the expected number of edges which \emph{remain} (are not contracted this iteration) is at most $2m D^{-1/2}$, under random choice of $h\in\mathcal H$. By the probabilistic method, there must be some $h$ for which at most this many edges remain, and we will pick such an $h$ to advance to the next iteration.

So, in each sequential iteration we reduce the number of edges by a factor of $2 D^{-1/2}$. Therefore, after $O(\log_D n)$ iterations, we have no edges remaining, and we either have one supernode (in which case we output that the input graph was a single cycle) or two (in which case we output two cycles).

The running time is dominated by $O(\log_D n)$ sequential applications of $A'$. Since $A'$ runs in $o(\log D)$ rounds, this is $o(\log n)$ rounds in total. The space usage is dominated by $n^{o(1)}$ parallel applications of $A'$, which in turn use $O(n^2)$ parallel instances of $A$. So, we use $O(n^\alpha)$ local space and $O(n^{2+\beta+o(1)})$ global space.
\end{proof}
%---------------------------------------------------------------------------------------------------------------------------------------------------------


%---------------------------------------------------------------------------------------------------------------------------------------------------------


%\bibliographystyle{plain}
%\bibliographystyle{alpha}
%\bibliography{derand+}
%\bibliography{ref}



==> comp-stab-def.tex <==



\subsection{Problems with GKU definition} 
\paragraph{Component stable-outputs must not depend on exact value of $n$}
Consider the following problem: each node should 


\paragraph{Randomness must be constrained}
\paragraph{Success probability must not depend on input size}
Consider a component-stable MPC algorithm $A$ for an locally-checkable (or component-stable, i.e., where a node's output can be verified by seeing its connected component) problem, running on a $n$-node graph. Under the GKU definition, this algorithm must produce a valid output for each node in the graph with probability at least $1-\frac 1n$. 

We now add $N$ disconnected nodes to the input graph. $A$'s output on each of the original nodes must be unchanged, since they are in an unchanged connected component. However, $A$ must succeed on the new graph with probability at least $1-\frac{1}{n+N}$. Since the problem is component-stable, the probability that $A$ succeeds on all of the nodes of the original graph is at least as high as the probability that it succeeds on the whole graph, i.e., $1-\frac{1}{n+N}$. So, $A$ must succeed on the original graph with probability at least $1-\frac{1}{n+N}$, and since we can set $N$ arbitrarily high, must therefore succeed with certainty.

So, a definition of component-stability in which success probability depends on the size of the input graph does not allow algorithms with probabilistic success guarantees.

\subsection{Algorithm Definitions}


\paragraph{Randomized}
Input: Unique IDs, value $N$, $\Delta$, $N^\cs$ random bits

Correct output: If $N^\ce \le n\le N$, then with probability at least $1-\frac 1N$, correct output at every node.

Component-stable output: $v$'s output depends only on $v$'s ID, IDs of $v$'s component, randomness, $N$.

\paragraph{Deterministic}
Input: Unique IDs, value $N$?, $\Delta$

Correct output:  If $N^\ce \le n\le N$, correct output at every node.

Component-stable output: $v$'s output depends only on $v$'s ID, IDs of $v$'s component, $N$?

\paragraph{LOCAL, randomized}
Extra input: Unique IDs, value $N$, exact $\Delta$, unlimited shared random bits

Correct output:  If $N^\ce \le n\le N$, correct output at every node with probability at least $1-\frac 1N$.

\paragraph{LOCAL, deterministic}
Extra input: Unique IDs, value $N$, exact $\Delta$.

Correct output:  If $N^\ce \le n\le N$, correct output at every node with probability.


We will set $\alpha = \kappa\sparam$, where $\sparam$ is the MPC space parameter and $\kappa$ is a sufficiently small constant.
\junk{
We now formalize the process of probability amplification in MPC under this definition:


\begin{lemma}
Given a randomized $T(N,\Delta)$-round MPC algorithm $A_{MPC}$, for a problem $P$ which can be deterministically verified in $O(T(N,\Delta))$ rounds, which succeeds with probability $\frac 12$, taking as input $N$, $\Delta$, and a random seed of $N^\cs$ bits, we can generate an algorithm $A_{MPC}$ which instead takes $N^{O(1)}$ random bits and succeeds with probability at least 
\end{lemma}

\begin{proof}
We create $N^c$ concurrent copies of the input graph, on disjoint groups of machines. Machines know which group they belong to 

The random seed also is divided into $N^c$ strings of equal length, each of which is assigned to a group of machines. Groups of machines then simulate $A_{MPC}$ on their copy of the input graph using the random seed assigned to them (and the same input values for $N$ and $\Delta$). Node IDs in each copy of $G$ are also kept the same, but these multiple copies of nodes with identical IDs do not get conflated because machines only communicate with others in their group during the simulation.

Each group of machines then runs the verification algorithm on the output of their simulation. If any of the simulations was successful, 
\end{proof}}
\subsection{Sensitivity}

Each edge ${u, w}$ of the input graph is labeled by the set of IDs $\{ID(u),ID(w)\}$. We consider MPC inputs to be given with each edge assigned to a machine sharing the edge's identifier. The algorithm also receives the value $N$, and $N^c$ random bits, as input.

\begin{definition}
	[$(r, \eps)$-Sensitive MPC Algorithm]
	
For an integer $r \ge 0$ and some $\eps > 0$, an MPC
algorithm A for some graph problem is called $(r, \eps)$-sensitive w.r.t. two $r$-hop-isomorphic centered
graphs $G = (V, E)$ and $G' = (V', E')$ with centers $v \in V$ and $v'\in V'$ if the following is true.

We consider two dependent runs of A, one on $G$ and one on $G'$. In both runs, each node in the isomorphic r-hop neighborhoods $G[N_r(v)]$ and $G'[N_r(v')]$ are assigned the same uniformly chosen random IDs from $[N^c]$. (REWORD) All the remaining nodes, in $G$ and $G'$, are assigned
independently and uniformly chosen random IDs from the ID space of $[N^c]$. 

Then, if the MPC algorithm A is run on $G$ and $G'$ with the random seed, the probability that the two centers $v$ and $v'$ output different values is at least $\eps$ (the probability is taken over
the choice of random IDs and the shared randomness).
\end{definition}

\begin{lemma}
Let $P$ be a graph problem for which there is no $T(K,\Delta)$-round LOCAL algorithms that solves $P$ on maximum degree $\Delta$, with valid input estimate $K$, from a hereditary family $\mathcal G$, with probability at least $1-\frac 1K$.

Then, for every $N$ with $N^\alpha \le K \le N$, for any MPC algorithm that solves $P$ on $\mathcal G$, given valid input estimate $N$, there are two $T(K,\Delta)$-hop-indistinguishable centered graphs $G,G'\in \mathcal G$ with $K$ nodes and maximum degree $\Delta$, such that $A_{MPC}$ is $(T(K,\Delta), \eps)$ sensitive with respect to $G,G'$.

\end{lemma}

\begin{proof}
Denote $R=T(K,\Delta)$. Let us assume that there are not two centered graphs $G$ and $G'$ with $K$ nodes and maximum degree $\Delta$ such that the given MPC algorithm $A_{MPC}$ is $(R, \eps)$-sensitive w.r.t. $G$
and $G'$. We use this fact to construct a $R$-round randomized LOCAL algorithm $A_{LOCAL}$ to solve $P$ on graphs with valid size estimate $K$ with probability at least $1 - 1/K$, which is a contradiction to the assumption of the lemma that no such algorithm exists

Let $\delta  > 0$ be an arbitrarily chosen constant. We define $K := N^{\kappa\delta}$ for a sufficiently
small constant $\kappa > 0$ and we define $\eps := N^{-\delta}$. 

The input for $A_{LOCAL}$ is then a graph $H$ with 
\begin{itemize}
	\item a value $K$
	\item $\Delta$, the maximum degree of $H$,
	\item unlimited shared randomness
\end{itemize}

We require $A_{LOCAL}$ to give a correct output at every node with probability at least $1-\frac 1K$ if the (unknown) number of nodes in , denoted $n_H$, satisfies $n_H\le K\le n_H^\ce$. Otherwise, we place no requirements on its output.

We construct $A_{LOCAL}$ as follows: first, $A_{LOCAL}$ divides its random input $\mathcal S$ into three parts, $\mathcal S_1$, $\mathcal S_2$, and $\mathcal S_3$, as follows: 

\begin{itemize}
	\item $\mathcal S_1$ consists of $N^VVV$ bits and is allocated to provide a seed for simulating $A_{MPC}$
	\item $\mathcal S_2$ is used to give a uniformly random function $f:ID(A_{LOCAL}) \rightarrow [K^{3/\alpha}]$, mapping IDs from the ID space of $A_{LOCAL}$ to new uniformly random IDs in $[K^{3/\alpha}]$.
\junk{	\item $\mathcal S_3$ is allocated to randomly extend graphs VVV}

\end{itemize}

\junk{, uses $\mathcal S_2$ to randomly extend this to a $K$-node graph, uses $\mathcal S_3$ to map all IDs to uniformly random IDs in $[K^{3/\alpha}]$, and then simulates $A_{MPC}$ on this graph, with input estimate $N$, $\Delta$, and random seed $\mathcal S_1$.}

We now proceed in a similar fashion to the proof of Lemma 3.1 of \cite{GKU19}. Each node $v$ collects its $R$-radius ball $B_R(v)$. It then considers the family $\mathcal H_v$ of all $K$-node graphs centered at $v$, with IDs from the ID space of $A_{LOCAL}$, that are $R$-hop-identical to $B_R(v)$, i.e. the set of possible inputs to $A_{LOCAL}$ for which $v$ would see $B_R(v)$ as its $R$-radius ball. For any graph $G\in \mathcal H$, we then run $A_{MPC}$ on $G$, with input estimate $N$, $\mathcal S_1$ as the random seed, the value of $\Delta$, and IDs given by applying the function $f$ to the IDs of $G$. We then denote $OUT_{\mathcal S, G} (v)$ to be the output given by $A_{MPC}$ for the node $v$.

Then, we set

\[f_{LOCAL} (I) := \arg \max_{x\in \{1,\dots,\ell\}} |\{G\in \mathcal H_v: OUT_{\mathcal S, G} (v)=x \}|\enspace.\]

\paragraph{Correctness of the LOCAL algorithm}
Let $\mathcal I$ be the set of possible inputs $(B_R(v), \mathcal S)$. For an
input $I \in mathcal I$ and a pair of graphs $H_a, H_b \in H_v$, we define $P_{a,b}(I) := \Prob{}$
x=1 pa,x(I)· pb,x(I), which is the
probability that when running the above process on graphs Ha and Hb with input I, the centers of Ha
and Hb output the same value
 
Assume that we are given a labeled
$R$-hop neighborhood, which is given as a centered graph $H$ of radius at most $R$, where each node
of $H$ is labeled with a unique ID. Let $v_H$ be the center node of the centered graph $H$. Further,
let $\mathcal H$ be the family of all $K$-node centered graphs that are $R$-hop-isomorphic to $H$. That is, $\mathcal H$ is
the set of centered graphs, where the $R$-hop neighborhood of the center is equal to $H$ (without the
labels). We use the short notation ID(H) for the given assignment of IDs to H and we call the triple
(ID(H), S0, S1) the input of the LOCAL algorithm.
Let H = H1, . . . , Hq be an enumeration of all graphs in H. W.l.o.g., assume that the possible
set of output labels of a node are $L := \{1,\dots , \ell\}$ for some $\ell\ge 2$. For each graph Ha, we compute a
probability distribution over the ` possible output labels by evaluating the following random process.
We first assign a uniformly random ID to each node $u \in Ha$ that is not in the R-hop neighborhood
of the center node $v$ of $Ha$. That is, we assign a uniformly random ID to each node of Ha that is not
in H and thus does not have an ID assigned yet. Now, we deterministically compute an output label
for the center node $v$ as follows. Given the assignment of IDs, we then run the MPC algorithm AMPC with the second shared random bit string S1. Note that after fixing the input I = (ID(H), S0, S1), and the random IDs of
the nodes that are not in H, AMPC is a deterministic algorithm. For each output label $x \in{1, \dots \ell},$
we define $pa,x(I)$ as the probability that node v outputs label $x$. We set
\end{proof}

%---------------------------------------------------------------------------------------------------------------------------------------------------------


%---------------------------------------------------------------------------------------------------------------------------------------------------------





==> complete-conditionalLBproof.tex <==
Consider a graph problem $\mathcal{P}$ that has a $D=T(n)$-round lower bound in the randomized LOCAL model with shared randomness. Suppose that $T(n)\leq \log^{\gamma}n$ for some constant $\gamma \in (0,1)$ and that there is an $o(\log D)$-round \textbf{component-stable} MPC algorithm $\mathcal{A}$ that solves $\mathcal{P}$ using $n^{\alpha}$ local space. We will show that there is an MPC algorithm with local memory $n^{\beta}$ that solves the $D$-diam $s$-$t$ connectivity in $o(\log D)$ rounds. 
\\ \\
\noindent \textbf{Sensitivity:} By Lemma 3.1, there exists two $D=t(n)$-hop isomorphic centered graphs $G,G'$ of size less than $n^{\delta}$ such that $\mathcal{A}$ is $(t(n), n^{1/\delta})$-sensitive w.r.t $G$ and $G'$. Let $v,v'$ be the centers of these two $D=t(n)$-hop isomorphic centered graphs. By Def. 3.1, the sensitivity property implies the following. Consider two independent runs of $\mathcal{A}$ on $G,G'$. In both runs, the edges of $G[N_D(v)]$ and $G'[N'_D(v)]$ are mapped to the same machines. This is done by using a shared seed $\mathcal{SR}_0$ to assign the \emph{same} random IDs to the nodes in $G[N_D(v)],G'[N'_D(v)]$, and then map the IDs of the edges in these graphs to random machines based on their IDs (i.e., the ID of an edge is a pair of its endpoint IDs). The remaining nodes of $G \setminus G[N_D(v)]$ and $G \setminus G[N_D(v)]$ are given independent IDs and sent to independent machines using a shared seed $\mathcal{SR}_0$. The algorithm is then applied on both $G,G'$ using the shared seed $\mathcal{SR}_1$. The sensitivity of $\mathcal{A}$ implies that the probability (over the shared seeds) that $v,v'$ have a different outputs in both runs is at least $\epsilon=n^{1/\delta}$. 
\begin{equation}\label{eq:sensitivity}
Pr_{\mathcal{SR}_0,\mathcal{SR}_1}[out_{\mathcal{A}}(v,G,\mathcal{SR}_0,\mathcal{SR}_1)\neq out_{\mathcal{A}}(v,G',\mathcal{SR}_0,\mathcal{SR}_1)]\geq \epsilon~.
\end{equation}

\emph{Remark:} It seems that one should require that both the graphs $G[N_{D+1}(v)]$ and $G'[N'_{D+1}(v)]$ are \emph{connected}. This seems to hold as the local LBs are usually obtained on connected graphs. 
\\
\noindent\textbf{Component Stability:} Since  $\mathcal{A}$ is component stable, it holds that in \emph{every} graph, the output of $v$ depends \emph{deterministically} on the IDs and the edge distribution (to machines) of all edges in its components, and the shared seed $\mathcal{SR}$. For every graph $H$ and node $u \in V(H)$, let $H_u$ be the connected component of $u$ in $H$, then:

\begin{equation}\label{eq:stability}
out_{\mathcal{A}}(u,H)=f_{\mathcal{A}}(IDs(H_u), \mathcal{SR})~.
\end{equation}
This in particular implies, that if there are two runs of $\mathcal{A}$ on different graphs $H,H'$ where $H_v=H'_v$ and when using the \emph{same} shared seed (in both runs while all edges of $H_v=H'_v$ are assigned to the same machines), the output of $v$ in both runs is the same (with probability $1$).
\\ \\
\noindent\textbf{Solving $D$-diam $s$-$t$ connectivity using Alg. $\mathcal{A}$:} The input graph $F$ to the connectivity problem consists of two special nodes $s$ and $t$. It is required to say YES only if $s$ and $t$ are the \emph{endpoints} of a path of length at most $D$. 

Throughout we assume that $n^{\delta}$ is small w.r.t to the local memory of the machines.
We describe an algorithm $\mathcal{B}$ that has the following property. If $s$ and $t$ are indeed endpoints of such a path then $s$ outputs YES w.p. $1/n^{\delta}$. Otherwise, $s$ outputs NO w.h.p. This algorithm can be then boosted to provide the final algorithm. Consider the algorithm $\mathcal{A}$ for problem $\mathcal{P}$, all nodes know the centered graphs $G,G'$ for which it is sensitive. They will let $s$ simulate the centered nodes $v,v'$. %and the node $t$ will be mapped to some unique node $t^*$ in $N_D(v)$.
Algorithm $\mathcal{B}$ attempts to simulate $\mathcal{A}$ on graphs that are \emph{related} to $G,G'$ in even and odd steps respectively. The only participating nodes in the input graph $F$ are the nodes $s,t$ and all nodes with degrees exactly two. The machine of each participating node will define a subset of edges and send them to designated machines in $[n,poly(n)]$. 
The node $s$ samples a  value $\ell \in [1,D]$ uniformly at random with the purpose of fixing the length of the $s$-$t$ paths (in YES instances) to be exactly $D$. Each node $u$ with degree $2$ picks a BFS layer $i$ uniformly at random in $[1,D]$ and exchange this number with its two neighbors. The node $u$ will \emph{simulate} layer $i$ (as will be explained next) only if its two neighbors $u',u''$ pick the layers $i-1,i+1$ respectively. 
Let $L_{j}=\{w_{1,j}, \ldots, w_{k_j,j}\}$ be the IDs of the layer $j$ in the BFS tree of $v$ in $G,G'$ for every $j \in [1,D]$. The IDs of the nodes in $L_{j}$ can be determined using the shared random seed known to all nodes. 

We now restrict attention to all validated nodes, namely, $s,t$ and all nodes whose BFS layer guess  is valid w.r.t their neighbors. These nodes (more accurately, the machines storing these nodes) will collectively define two graphs $\widehat{G}^0$ and $\widehat{G}^1$ to be used in even and odd steps respectively. 
Each validated node $u$ whose layer guess is $i$, renames the nodes in layer $i$ by $L^u_{i}=\{w_{u,1,i}, \ldots, w_{u,k_i,i}\}$. This indicates that $u$ "owns" these nodes. Since the nodes in layer $i$ have only edges in $G,G'$ to layers $i-1,i,i+1$, and since $u$ knows the graphs $G,G'$ and its corresponding neighbors $u',u''$ it can define the IDs of all edges incident to $L^u_{i}$ in $G,G'$. For example, any edge $(w_{a,i}, w_{b,i+1})$ where $w_{a,i} \in L_i$ and $w_{b,i+1} \in L_{i+1}$ will be mapped by $u$ to an edge $(w_{u,a,i}, w_{u'',b,i+1})$. The \emph{machine} holding $u$ can then compute all edges incident to $L^u_i$ in $\widehat{G}^0$ and $\widehat{G}^1$. For every $i \in [0,D]$, the random IDs of these nodes and the edge distribution are the same in both $\widehat{G}^0$ and $\widehat{G}^1$ and defined based on the shared seed. For simplicity, all these edges be assigned on machines in $[n,poly(n)]$. This code is applied for every vertex with degree exactly $2$ (including those lying on the $\ell$-length path added virtually by $s$). 

Finally, the node $t$ have different contributions to $\widehat{G}^0$ and $\widehat{G}^1$. 
The machine storing $t$ will pick independent IDs to all nodes in $G\setminus G[N_D(v)]$ and to nodes in $G'\setminus G[N_D(v)]$ using the shared seed. Specifically, we will have $L^{0,t}_j$ (resp., $L^{1,t}_j$) for $j \geq D$ be the layer $j$ in $G$ (resp., in $G'$). Note that $L^{0,t}_D=L^{1,t}_D$ as they are part of the $D$-hop ball of $v,v'$ in $G,G'$. For every $j\geq D+1$, the IDs of the nodes $L^{0,t}_j, L^{1,t}_j$ (and their corresponding edges in $G,G'$) are mapped independently using the shared seed. 
Again, the edges will be distributed on machines in $[n,poly(n)]$. In odd step (resp., even), $\mathcal{A}$ is applied on $\widehat{G}^0$ (resp., $\widehat{G}^1$). The output of $s$ is set to YES iff the output values of $v,v'$ are different in these two applications. It is then required to show that in a YES instance, $s$ outputs YES with prob. $1/n^{\delta}$ and in a NO-instance it outputs NO with high probability. The probability is over the shared seed. 

\begin{observation}\label{obs:given-graph}
\begin{description}
\item{(i)}
For every positive instance with bad guesses as well as for every negative instance, there is an $i \in [0,D]$ such that $\widehat{G}^0_v=\widehat{G}^1_v$ and\footnote{Recall that $\widehat{G}^0_v$ indicates the connected component of $v$ in $\widehat{G}^0$.} these graphs are isomorphic to $G[N_i(v)]$ and $G'[N_i(v)]$. 
%In addition, any node corresponding to $t$ in $\widehat{G}^0,\widehat{G}^1$ is not in the same component of $v$ in these graphs. 
\item{(ii)} For every positive instance with the correct guesses, $\widehat{G}^0_v$ is isomorphic to $G_v$ and $\widehat{G}^1_{v'}$ is isomorphic to $G'_{v'}$.
\end{description}
\end{observation}
\begin{proof}
(i) Consider first the case of positive instance with bad guesses. Let $i$ be the first layer that is not simulated by a node on the $s$-$t$ path. We have that $i\leq D$. Thus, all layers of $0,\ldots, i-1$ are simulated by the first $i$ nodes on the $s$-$t$ path. 
As a result, Since all these layers are mapped to the \emph{same} node and edge IDs in both $\widehat{G}^0_v,\widehat{G}^1_v$ the claim holds. (This holds as only the nodes of layers $\geq D+1$ are mapped to distinct IDs by $t$ in $\widehat{G}^0,\widehat{G}^1$.

Now consider the case of a NO instance. In case where the guesses along the path of $s$ are incorrect (i.e., do not sum up to a path of length $D$), the argument is as above. In the case where the guesses are indeed correct along the path of $s$ (i.e., we have length exactly $D$ and consecutive layer guesses), then all the $D+1$ layers are simulated by the nodes of this $s$-path. Since $t$ is not on that path, the nodes that it simulates are not in the connected component of $s$ in both $\widehat{G}^0,\widehat{G}^1$. Thus, the connected component of $v',v$ in both $\widehat{G}^0,\widehat{G}^1$ will be isomorphic to $G[N_D(v)]$ and  $G'[N_D(v)]$ as desired. 

(ii) Finally consider a YES instance with the right guesses. In this case, \emph{every} layer of the BFS tree of $v,v'$ in $\widehat{G}^0_v,\widehat{G}^1_{v'}$ is simulated in odd and even steps respectively, and thus the claim holds. 
\end{proof}


\begin{claim}
\begin{description}
\item{(a)} For every positive instance with bad guesses as well as for every negative instance, the output of $s$ in odd and even steps are the same (when using same shared seeds).\\ 

\item{(b)} For every positive instance with correct guesses, the output of $s$ in odd and even steps is distinct with probability $n^{\delta}$.
\end{description}
\end{claim}
\begin{proof}
(a) By Obs. \ref{obs:given-graph}(i), it holds that the connected components of $v$ in both graphs $\widehat{G}^0$ and $\widehat{G}^1$ are the same. Since the IDs of the nodes and the random assignment to machines are based on the same seed in both runs of $\mathcal{A}$ on $\widehat{G}^0$,$\widehat{G}^1$  and using the same shared seed for the simulation on these graphs, by the component stability of $\mathcal{A}$ (Eq. (\ref{eq:stability})) we have the the output of $v,v'$ in both runs are the same. Concluding that $s$ outputs NO. Note that here we only use the component stable property.

(b) By Obs. \ref{obs:given-graph}(ii), we have that $\widehat{G}^0_v$ is isomorphic to $G_v$, and in addition $\widehat{G}^1_{v'}$ is isomorphic to $G'_{v'}$. Since $\mathcal{A}$ is $(D,\epsilon)$ sensitive on $G,G'$ and since it is \emph{also} component stable, we have that it is $(D,\epsilon)$ sensitive on $G_v,G'_{v'}$. 
In both simulations on $\widehat{G}^0_v$ and $\widehat{G}^1_{v'}$ the edges of the $D$-ball around $v,v'$ are given same IDs and have the same distribution over the machines, while all other edges (outside the $D$-ball) in $\widehat{G}^0_v,\widehat{G}^1_{v'}$ are given independent IDs. Since $\mathcal{A}$ is $(D,\epsilon)$ sensitive on $G_v,G'_v$, it is also $(D,\epsilon)$-sensitive on their isomorphic copies $\widehat{G}^0_v$ and $\widehat{G}^1_v$ where $\epsilon$ is based on the shared seed used in these simulations. Thus, by Eq. (\ref{eq:sensitivity}), w.p at least $\epsilon$, the outputs of $v$ and $v'$ are distinct and consequently $s$ outputs NO.
\end{proof}



==> complexity-classes.tex <==
%\subsection{Complexity Classes}

In this section we define the complexity classes for \MPC considered in this paper. We consider the \MPC model described in Section \ref{sec:intro}, where each machines has $S$ words of space and $M$ denotes the number of machines. Since we normally focus on the case $S = n^{\delta}$ for some positive constant $\delta$, $0 < \delta < 1$, we will parameterize the complexity classes with respect to the local space to be of the form $n^{\gamma}$ for $0 < \gamma < 1$, and the number of machines to be $n^{\kappa}$ for $\kappa > 0$.\Artur{Or we want to state explicitly that $\kappa \ge 1$?}

We will consider only graph problems\Artur{I feel, it's OK to focus on graphs only. Do you agree?}. Let $\mathcal{G}$ be the collection of all input graph instances. We say that an \MPC algorithm $\mathcal{A}$ has round complexity $T(n)$ with local space $S(n)$ on $M(n)$ machines, if for any $n \in \mathbb{N}$, for any input instance on $n$ vertices, it performs at most $T(n)$ rounds on \MPC with local space $S(n)$ and $M(n)$ machines. A deterministic algorithm $\mathcal{A}$ solves a problem $\mathcal{P}$ if for any input instance $\mathcal{G}$ it returns a correct solution for $\mathcal{P}$ (e.g., for decision problem, it is a correct YES or NO). A randomized algorithm $\mathcal{A}$ solves a problem $\mathcal{P}$ with probability $1-p(n)$, $0 \le p(n) \le 1$, if for any input instance $G \in \mathcal{G}$ with $n$ vertices, it returns a correct solution for $\mathcal{P}$ with probability at least $1-p(n)$. (For the sake of simplicity, we focus on Monte Carlo randomized algorithms, which have fixed time complexity but may have some probability $1-p$ to err and produce an inadmissible output.)

We focus on upper bound round complexity, local space, global space, and success probability which depend only on the number $n$ of the graph's vertices in the input instance $\mathcal{G}$.\Artur{Here in the source file are definitions parameterized wrt $S$ and $M$ (require some polishing).}
%
\junk{
%
\begin{definition}[\textbf{\MPCDetNonStable}]
Denote by $\MPCDetNonStable(T(n),\alpha,\beta)$ the class of all graph problems $\mathcal{P}$ solvable by a deterministic \MPC algorithm $\mathcal{A}$, such that for some positive constant $c$, algorithm $\mathcal{A}$ has round complexity $c \cdot T(n)$ with local space $c \cdot n^{\alpha}$ and global space $c \cdot n^{\beta}$.\Artur{As you can see, here I want to suppress constant factors in the runtime and storage.}
\end{definition}

\begin{definition}[\textbf{\MPCDetStable}]
Denote by $\MPCDetStable(T(n),\alpha,\beta)$ the subclass of $\MPCDetNonStable(T(n),\alpha,\beta)$ restricted to component-stable algorithms (cf. Section \ref{subsec:alg-def}). That is, $\MPCDetStable(T(n),\alpha,\beta)$ is the class of all graph problems $\mathcal{P}$ solvable by a deterministic \MPC component-stable algorithm $\mathcal{A}$, such that for some positive constant $c$, algorithm $\mathcal{A}$ has round complexity $c \cdot T(n)$ with local space $c \cdot n^{\alpha}$ and global space $c \cdot n^{\beta}$.
\end{definition}

\begin{definition}[\textbf{\MPCRandNonStable}]
Denote by $\MPCRandNonStable(T(n),p(n),\alpha,\beta)$ the class of all graph problems $\mathcal{P}$ solvable with probability $p(n)$ by a randomized \MPC algorithm $\mathcal{A}$, such that for some positive constant $c$, algorithm $\mathcal{A}$ has round complexity $c \cdot T(n)$ with local space $c \cdot n^{\alpha}$ and global space $c \cdot n^{\beta}$.
\end{definition}

\begin{definition}[\textbf{\MPCRandStable}]
Denote by $\MPCRandStable(T(n),p(n),\alpha,\beta)$ the subclass of the class $\MPCRandNonStable(T(n),p(n),\alpha,\beta)$ restricted to component-stable algorithms (cf. Section \ref{subsec:alg-def}). That is, $\MPCRandStable(T(n),p(n),\alpha,\beta)$ is the class of all graph problems $\mathcal{P}$ solvable with probability $p(n)$ by a randomized \MPC component-stable algorithm $\mathcal{A}$, such that for some positive constant $c$, algorithm $\mathcal{A}$ has round complexity $c \cdot T(n)$ with local space $c \cdot n^{\alpha}$ and global space $c \cdot n^{\beta}$.
\end{definition}
%
}
%
Since our main focus is to study the regime of $n^{1-\Omega(1)}$ local memory and a polynomial number of machines, we consider the following definitions.

\begin{definition}[\textbf{\MPCDetNonStable}]
Denote by $\MPCDetNonStable(T(n))$ the class of all graph problems for which there is a deterministic \MPC algorithm $\mathcal{A}$, such that for some positive constant $c$, algorithm $\mathcal{A}$ has round complexity $c \cdot T(n)$ on an \MPC with local space $n^{1-\Omega(1)}$ on $\poly(n)$ machines.\Artur{As you can see, here I want to suppress constant factors in the runtime and failure probability.}
%for some positive constant $\delta < 1$ and arbitrary large constant $c$, algorithm $\mathcal{A}$ has round complexity $c \cdot T(n)$ on an \MPC  with local space $c \cdot n^{\delta}$ on a polynomial (in $n$) number of machines.\Artur{As you can see, here I want to suppress constant factors in the runtime. One could also possibly replace $c \cdot n^{\delta}$ by $n^{1-\Omega(1)}$.}
\end{definition}

\begin{definition}[\textbf{\MPCDetStable}]
Denote by $\MPCDetStable(T(n))$ the subclass of $\MPCDetNonStable(T(n))$ restricted to component-stable algorithms. That is, $\MPCDetStable(T(n))$ is the class of all graph problems for which there is a deterministic component-stable \MPC algorithm $\mathcal{A}$, such that for some positive constant $c$, algorithm $\mathcal{A}$ has round complexity $c \cdot T(n)$ on an \MPC with local space $n^{1-\Omega(1)}$ on $\poly(n)$ machines.
\end{definition}

\begin{definition}[\textbf{\MPCRandNonStable}]\Artur{If we wanted, we could stick to some more specific $p(n)$, for example, a constant or $1-1/n$.}
Denote by $\MPCRandNonStable(T(n),p(n))$ the class of all graph problems $\mathcal{P}$ for which there is a randomized \MPC algorithm $\mathcal{A}$, such that for some positive constant $c$, algorithm $\mathcal{A}$ solves $\mathcal{P}$ with probability $1 - c \cdot p(n)$ and has round complexity $c \cdot T(n)$ on an \MPC with local space $n^{1-\Omega(1)}$ on $\poly(n)$ machines.
\end{definition}

\begin{definition}[\textbf{\MPCRandStable}]
$\MPCRandStable(T(n),p(n))$ is the subclass of $\MPCRandNonStable(T(n),p(n))$ restricted to component-stable algorithms. That is, $\MPCRandStable(T(n),p(n))$ is the class of all graph problems $\mathcal{P}$ for which there is a randomized component-stable \MPC algorithm $\mathcal{A}$, such that for some positive constant $c$, algorithm $\mathcal{A}$ solves $\mathcal{P}$ with probability $1 - c \cdot p(n)$ and has round complexity $c \cdot T(n)$ on an \MPC with local space $n^{1-\Omega(1)}$ on $\poly(n)$ machines.
\end{definition}

Clearly, for any functions $T(n)$ and $p(n)$, we have $\MPCDetStable(T(n)) \subseteq \MPCDetNonStable(T(n))$ and $\MPCRandStable(T(n),p(n)) \subseteq \MPCRandNonStable(T(n),p(n))$. We can prove the following:
%In the regime of \MPC with local space $n^{1-\Omega(1)}$ on $\poly(n)$ machines, we have the following claims.

\begin{claim}
There is some function $T(n)$\Artur{Give some values/function.} such that
%
\begin{align*}
    \MPCDetStable(T(n)) \subsetneqq \MPCDetNonStable(T(n))
	\enspace.
\end{align*}
\end{claim}

\begin{claim}
There are some functions $T(n)$ and $p(n)$, $0 < p(n) < 1$,\Artur{Give some values/function. Does it hold for some $p(n)$ or for all $p(n)$?} such that
%
\begin{align*}
    \MPCRandStable(T(n),p(n)) \subsetneqq \MPCRandNonStable(T(n),p(n))
	\enspace.
\end{align*}
\end{claim}

Further, we notice that $\MPCDetNonStable = \MPCRandNonStable$ if we allow ???\Artur{This is about these uniform vs. non-uniform algorithms.}

$\poly(n)$ global memory and local problems, we get that:\Artur{Do we want to state these as claims/theorem?}
%
\begin{align*}
	\MPCDetStable \quad \subsetneqq \quad \MPCDetNonStable \quad = \quad \MPCRandNonStable \quad \supsetneqq \quad \MPCRandStable
	\enspace.
\end{align*}

In addition:
%
\begin{align*}
	\MPCDetStable \quad \supsetneqq \quad \MPCRandStable
	\enspace.
\end{align*} 

==> lift.tex <==
%---------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{Conditional \MPC Lower Bounds from \LOCAL}
%\label{sec:lb-LOCAL->MPC}

In this section, we present a revised framework lifting unconditional lower bounds from the \LOCAL model to conditional lower bounds for low-space component-stable \MPC algorithms, correcting in \Cref{thm:lb} the analysis of Ghaffari et al. \cite{GKU19}.
\Peter{To myself: align this with the new paragraph in section 2}

While on a high level, our analysis follows closely the approach from \cite{GKU19}, our arguments diverge in several \emph{subtle} but \emph{crucial} places. On a technical level, we rely on the central but also quite subtle notions of \emph{replicable graph problems}, \emph{normal graph families}, \emph{$(D, \eps, n, \Delta)$-sensitive \MPC algorithms}, and a revised definition of \emph{component stability} (see Definition \ref{def:component-stable-algorithms}). The two major reasons behind these changes are:
%
\begin{itemize}
\item to make the arguments robust against the issues we have identified concerning component-stability, and incorporate the definitional changes that these issues necessitated, and
\item to extend the arguments to include lower bounds against \emph{deterministic algorithms}, and lower bounds with \emph{dependency on maximum input degree $\Delta$}.
\end{itemize}

As mentioned above, on a high level, our arguments follow the line of the arguments from \cite{GKU19}, but some subtle details sketched above require us to revise the analysis. After introducing some useful notation in \Cref{subsec:basic-def}, we show in \Cref{subsec:sens} that in our setting, for $R$-replicable graph problems for normal graph families, lower bounds for \LOCAL algorithms imply the existence of some graphs which can be distinguished by component-stable \MPC algorithms only by relying on non-local information. Then, in \Cref{subsec:stconn}, we apply this non-locality to provide a conditional \MPC lower bound for component-stable \MPC algorithms for $O(1)$-replicable graph problems in our setting (for normal graph families). In particular, conditioned on the connectivity conjecture, our main result (\Cref{thm:lb}) states, informally, that for $O(1)$-replicable graph problems, any $T(N,\Delta)$-round lower bound in the \LOCAL model yields a $\Omega(\log T(N,\Delta))$-round lower bound for any low-space component-stable \MPC algorithm $\mathcal{A}_{\MPC}$. Furthermore, the claim holds for both randomized and deterministic algorithms.
%
%Finally, in \Cref{subsec:lb:applications} we apply our framework to conclude with a list of conditional lower bounds for several classical graph problems for any low-space component-stable \MPC algorithms.\Artur{\textcolor[rgb]{0.50,0.00,0.50}{Here (or/and somewhere else, in Intro?) we should have some discussion that some of these results have been claimed in \cite{GKU19}, but given the problems with their notion of component-stable algorithms these claims are \emph{XXXXX}. Furthermore, the novelty of our results include dependency on $\Delta$ and the results for deterministic \MPC algorithms.}}

%---------------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Basic definitions: \emph{normal graph families} and \emph{sensitive \MPC algorithms}}
\label{subsec:basic-def}

\begin{definition}
Two connected graphs $G = (V, E)$ and $G' = (V', E')$, with \emph{center} nodes $v \in V$ and $v'\in V'$ respectively, are \textbf{$D$-radius-identical} if the topologies and node IDs (but not necessarily names) of the $D$-radius balls around $v$ and $v'$ are identical.
\end{definition}

Our next definition (related to \cite[Definition~III.1]{GKU19}, though set up in our framework), formalizes the notion of \MPC algorithms depending on non-local information in the graph.

\begin{definition}[\textbf{$(D, \eps, n, \Delta)$-sensitive \MPC algorithms}]
\label{def:sensitive-MPC-algorithms}
For integers $D,n,\Delta \ge 0$ and some $\eps \in [0,1]$, a component-stable \MPC algorithm $\mathcal{A}$ for some graph problem is called \textbf{$(D, \eps, n,\Delta)$-sensitive} with respect to two $D$-radius-identical centered graphs $G = (V, E)$ and $G' = (V', E')$, with centers $v \in V$ and $v'\in V'$, if the probability (over choice of seed $\mathcal{S}$) that $\mathcal{A}(G, v, n, \Delta, \mathcal{S}) \ne \mathcal{A}(G', v', n, \Delta, \mathcal{S})$ is at least $\eps$.
\end{definition}

We can apply this definition also to deterministic component-stable algorithms. Since these do not depend on the random seed, any $(D, \eps, n, \Delta)$-sensitive deterministic  component-stable \MPC algorithm with $\eps > 0$ is $(D, 1, n, \Delta)$-sensitive.

As one final point of notation, in this section our arguments will often involve several different graphs. For clarity, for any graph $G$ we will denote by $n_G$ its number of nodes.

%---------------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{\LOCAL hardness yields indistinguishability of graphs locally}
\label{subsec:sens}

Our next lemma (cf. \cite[Lemma~III.1]{GKU19}) shows that a lower bound for a normal family for any \LOCAL algorithm for some $R$-replicable graph problem implies some useful property for any component-stable \MPC algorithm for that problem: to distinguish some graphs from that normal family one needs to rely on non-local information, in the sense of Definition~\ref{def:sensitive-MPC-algorithms}.

\begin{lemma}
\label{lem:sens}
For any $N, \Delta, R \in \nat$, let $\mathcal{P}$ be an $R$-replicable graph problem for which there is no $T(N,\Delta)$-round \LOCAL algorithm that solves $\mathcal{P}$ on graphs from some normal family $\mathcal{G}$ of maximum degree $\Delta$, with input size estimate $N$ (i.e., satisfying $n_H \le N \le poly(n_H)$), and with probability at least $1-\frac1N$.

Suppose there is a component-stable \MPC algorithm $\mathcal{A}_{\MPC}$ that solves $\mathcal{P}$ on all graphs $G \in \mathcal{G}$, with probability at least $1 - \frac{1}{n_G}$. Then, there are two $T(N,\Delta)$-radius-identical centered graphs $G, G' \in \mathcal{G}$ with at most $N$ nodes and maximum degree (exactly) $\Delta$, such that $\mathcal{A}_{\MPC}$ is $(T(N,\Delta), \frac{1}{4N^2},N^{R+2},\Delta)$-sensitive with respect to $G,G'$.

The same claim holds if the \LOCAL lower bound and algorithm $\mathcal{A}_{\MPC}$ are both \emph{deterministic}.
%
%For any $N,\Delta,R\in \nat$, let $P$ be a $R$-replicable graph problem for which there is no $T(N,\Delta)$-round \LOCAL algorithm that solves $P$ on graphs from some normal family $\mathcal{G}$ of maximum degree $\Delta$, with \Artur{What does it mean? Did we define the notion of \emph{valid input size estimate}? (BTW input is of size $\Theta(|V(G)|+|E(G)|)$, or maybe even $\Theta((|V(G)|+|E(G)|)\log(|V(G)|+|E(G)|))$ bits; is it what we want to have?)}a valid input size estimate $N$, and with probability at least $1-1/N$.
%
%Suppose there is a component-stable \MPC algorithm $\mathcal{A}_{\MPC}$ that solves $P$ on all graphs $G \in \mathcal{G}$, with probability at least $1 - \frac{1}{|V(G)|}$\Artur{I changed $1/n_G$ to $1/|V(G)|$; I feel it's better to avoid using $n_G$.}. Then, there are two $T(N,\Delta)$-radius-identical centered graphs\Artur{Define the notion of $D$-radius-identical centered graphs.} $G, G' \in \mathcal{G}$ with at most $N$ nodes and maximum degree (exactly) $\Delta$, such that $\mathcal{A}_{\MPC}$ is $(T(N,\Delta), \frac{1}{4N^2},N^{R+2},\Delta)$-sensitive with respect to $G,G'$.
%
%The same claim holds if the \LOCAL lower bound and algorithm $\mathcal{A}_{\MPC}$ are both \emph{deterministic}.
\end{lemma}

\begin{proof}
The proof is by contradiction. Denote $D = T(N,\Delta)$ and $\eps = \frac{1}{4N^2}$. Let us assume that there are no two $D$-radius-identical centered graphs $G, G' \in \mathcal{G}$ with at most $N$ nodes and maximum degree $\Delta$ such that the given \MPC algorithm $\mathcal{A}_{\MPC}$ is $(D, \eps, N^{R+2}, \Delta)$-sensitive with respect to $G$ and $G'$. We use this fact to construct a $D$-round randomized \LOCAL algorithm $\mathcal{A}_{\LOCAL}$ to solve $\mathcal{P}$ on graphs with valid size estimate $N$ with probability at least $1 - \frac1N$, which is a contradiction to the assumption of the lemma.

%(In what follows, for simplicity, for any graph $U$ we use notation $n_U$ to denote $|V(U)|$.)

\paragraph{Design of the \LOCAL algorithm.}

The input for $\mathcal{A}_{\LOCAL}$ is an unbounded random seed $\mathcal{S}$, a graph $H \in \mathcal{G}$, integers $N$, $\Delta$, and the assignment of the IDs to the nodes of $H$, such that:
%
\begin{itemize}
\item $N$ is the input size estimate, that is, $n_H \le N \le poly(n_H)$,
\item $\Delta$ is the maximum degree of $H$,
\item all IDs are in $[\poly(N)]$ and are component-unique.
\end{itemize}

\junk{
The input for $\mathcal{A}_{\LOCAL}$ is an unbounded random seed $\mathcal{S}$ and an arbitrary graph $H \in \mathcal{G}$ with:
%
\begin{itemize}
\item a valid input size estimate $N$ (i.e., $n_H \le N$),
\item component-unique IDs in $[\poly(N)]$,
\item maximum degree exactly $\Delta$.
\end{itemize}
}

For a fixed $H$, let us take an arbitrary node $v$ and describe how to determine $v$'s output under $\mathcal{A}_{\LOCAL}$, on a particular input $\mathcal{I} = \langle H, \mathcal{S} \rangle$. Node $v$ first collects its $D$-radius ball $B_D(v)$ in $H$. It then considers the family $\mathcal{H}_v$ of all graphs with at most $ N$ nodes, centered at $v$, with component-unique IDs from $[\poly(N)]$, and maximum degree $\Delta$ that are $D$-radius-identical to $B_D(v)$, i.e., the set of possible inputs to $\mathcal{A}_{\LOCAL}$ for which $v$ would see $B_D(v)$ as its $D$-radius ball. For each $G\in \mathcal{H}_v$, $v$ creates a \emph{simulation graph $\Gamma_G$} (cf. Definition \ref{def:replicable}) as follows: $\Gamma_G$ consists of $\lfloor \frac{N^{R+2}}{n_G} \rfloor \ge n_G^R$ disjoint copies of $G$. One of these copies is arbitrarily designated the \emph{``true'' copy}, and its nodes use the IDs of $G$ as their own IDs and names. All other copies use the same IDs, but as names they use arbitrary unique values in $[\poly(N)]$. We also add enough isolated nodes to raise the number of nodes to exactly $N^{R+2}$ (i.e., $N^{R+2} - n_G\lfloor \frac{N^{R+2}}{n_G} \rfloor < n_G$ isolated nodes), sharing the same arbitrary ID, and with arbitrary unique names, in $[\poly(N)]$.

In order to determine the output of $\mathcal{A}_{\LOCAL}$ at $v$, we will be running $\mathcal{A}_{\MPC}$ on the simulation graph $\Gamma_G$. For the supply of randomness, denote $\mathcal{S}'$ to be $\mathcal{S}$ curtailed to the length required by $\mathcal{A}_{\MPC}$, i.e., the first $\poly(N)$ bits. Since $\mathcal{A}_{\MPC}$ is component-stable, its output at $v$ on $\Gamma_G$, using seed $\mathcal{S}'$, is $\mathcal{A}_{\MPC}(G,v,N^{R+2},\Delta,\mathcal{S}')$.

Then, we set
%
\begin{align*}
    \mathcal{A}_{\LOCAL} (H,v,\mathcal{S}) &:=
    \arg \max_{x} |\{G\in \mathcal{H}_v: \mathcal{A}_{\MPC}(G,v,N^{R+2},\Delta,\mathcal{S}')=x \}|
    \enspace,
\end{align*}
%
i.e., $v$'s output label output by $\mathcal{A}_{\LOCAL}$ is that returned by the most $\mathcal{A}_{\MPC}$ simulations.

\paragraph{Correctness of the \LOCAL algorithm.}

We use our assumption that there are no two $D$-radius-identical centered graphs $G, G' \in \mathcal{G}$ with at most $N$ nodes and maximum degree $\Delta$ for which $\mathcal{A}_{\MPC}$ is $(D, \eps, N^{R+2}, \Delta)$-sensitive with respect to $G$ and $G'$. Hence, for any $G, G' \in \mathcal{H}_v$, with probability at least $1-\eps$ over choice of $\mathcal{S}$, $\mathcal{A}_{\MPC}(G, v, N^{R+2}, \Delta, \mathcal{S}')= \mathcal{A}_{\MPC}(G', v, N^{R+2}, \Delta, \mathcal{S}')$. In particular, since the actual input graph $H$ is certainly in $\mathcal{H}_v$,
%
\begin{align*}
    \mathbf E_{\mathcal{S}}\left[ \frac {|\{G\in \mathcal{H}_v:\mathcal{A}_{\MPC}(G,v,N^{R+2},\Delta,\mathcal{S}')\ne \mathcal{A}_{\MPC}(H,v,N^{R+2},\Delta,\mathcal{S}') \}|}{|\mathcal{H}_v|}\right]
        & \le
    \eps
    \enspace.
\end{align*}

Then, for the random seed $\mathcal{S}$, the probability that
%
\begin{align*}
    \frac {|\{G\in \mathcal{H}_v:\mathcal{A}_{\MPC}(G,v,N^{R+2},\Delta,\mathcal{S}') \ne \mathcal{A}_{\MPC}(H,v,N^{R+2},\Delta,\mathcal{S}') \}|}{|\mathcal{H}_v|}
        &\ge
    \frac12
    \enspace.
\end{align*}

is at most $2\eps$ by Markov's inequality. We therefore have
%
\begin{align*}
    \Prob{\mathcal{A}_{\LOCAL} (H, v, \mathcal{S}) =
        \mathcal{A}_{\MPC}(H, v, N^{R+2}, \Delta, \mathcal{S}')}
        &\ge
    1 - 2 \eps
    \enspace.
\end{align*}

Taking a union bound over all nodes $v \in V(H)$, we have that
%
\begin{align*}
    \Prob{\text{for all $v \in V(H)$: }
        \mathcal{A}_{\LOCAL} (H,v,\mathcal{S}) =
        \mathcal{A}_{\MPC}(H,v,N^{R+2},\Delta,\mathcal{S}')}
        &\ge
    1 - 2 N \eps
    \enspace.
\end{align*}

In this case, the overall output of $\mathcal{A}_{\LOCAL} (H, \mathcal{S})$ is equal to the output of $\mathcal{A}_{\MPC}$ on the true copy of $H$ when run on $\Gamma_H$ with seed $S'$. Since $\Gamma_H \in \mathcal{G}$ (as it is a disjoint union of members of $\mathcal{G}$, see Definition \ref{def:normal-graphs}), $\mathcal{A}_{\MPC}$ returns a valid output on $\Gamma_H$ with probability $1-1/n_{\Gamma_H} = 1- N^{-(R+2)}$. Note that $\Gamma_H$ is a disjoint union of at least $n_H^{R}$ copies of $H$ and fewer than $n_H$ extra isolated nodes. This satisfies the construction in the definition of $R$-replicability.\footnote{when $n_H \ge 2$; for $n_H \le 1$ Lemma \ref{lem:sens} is trivial since there can be no \LOCAL lower bounds on such graphs.} Since $\mathcal{A}_{\MPC}$ is component-stable, it must return the same output labeling in all copies of $H$ in $\Gamma_H$ (since they share the same topology and IDs), and likewise must return the same output label on all isolated nodes. So, the output labeling given on $\Gamma_H$ is of the form required in the replicability definition, and so $\mathcal{A}_{\MPC}$ returns a valid output on the true copy (and, indeed, on all copies) of $H$ in $\Gamma_H$.

Then, by a union bound, $\mathcal{A}_{\LOCAL}$'s output is correct with probability at least $1-2N\eps - N^{-(R+2)} \ge 1 - \frac1N$, reaching a contradiction to our assumption of a \LOCAL lower bound. This proves the randomized part of the lemma.

To prove the deterministic analogue, we perform exactly the same construction, except that $\mathcal{A}_{\LOCAL}$ does not have the random seed $\mathcal{S}$, and does not pass it to $\mathcal{A}_{\MPC}$. Since our algorithm $\mathcal{A}_{\LOCAL}$ is now deterministic, we have $\mathcal{A}_{\LOCAL}(H,v) = \mathcal{A}_{\MPC}(H,v,N^{R+2},\Delta)$ with certainty for all $v$, i.e., $\mathcal{A}_{\LOCAL}$'s output is identical to $\mathcal{A}_{\MPC}$'s output on an $N^{R+2}$-node graph containing $H$ as a connected component. Since $\mathcal{A}_{\MPC}$ is also deterministic, this is a valid output on $H$ with certainty. We have then constructed a deterministic \LOCAL algorithm solving $\mathcal{P}$, contradicting our initial assumption. So, we must instead have that $\mathcal{A}_{\MPC}$ is $(T(N,\Delta), 1,N^{R+2},\Delta)$-sensitive, and therefore, since it is deterministic, $(T(N,\Delta), 1,N^{R+2},\Delta)$-sensitive.
\end{proof}

%---------------------------------------------------------------------------------------------------------------------------------------------------------
%JUST FOR COMPARISON: THE OLD PROOF IS BELOW (commented)
\junk{
\begin{proof}
Denote $D = T(N,\Delta)$ and $\eps = \frac{1}{4N^2}$. Let us assume that there are no two centered graphs $G$ and $G'$ with $N$ nodes and maximum degree $\Delta$ such that the given \MPC algorithm $\mathcal{A}_{\MPC}$ is $(D, \eps, N^{R+2}, \Delta)$-sensitive with respect to $G$ and $G'$. We use this fact to construct a $D$-round randomized \LOCAL algorithm $\mathcal{A}_{\LOCAL}$ to solve $\mathcal{P}$ on graphs with valid size estimate $N$ with probability at least $1 - 1/N$, which is a contradiction to the assumption of the lemma.

The input for $\mathcal{A}_{\LOCAL}$ will be a graph $H$ with:
\begin{itemize}
	\item a valid input size estimate $N$ (i.e., $n_H\le N$),
	\item component-unique IDs in $[\poly(N)]$,
	\item maximum degree exactly $\Delta$.
\end{itemize}

$\mathcal{A}_{\LOCAL}$ also receives an unbounded random seed $\mathcal{S}$.

We now fix a node $v$ to consider, and describe how we determine $v$'s output under $\mathcal{A}_{\LOCAL}$, on a particular input $I=(\mathcal{S},H)$. Node $v$ first collects its $D$-radius ball $B_D(v)$ in $H$. It then considers the family $\mathcal{H}_v$ of all graphs with at most $ N$ nodes, centered at $v$, with component-unique IDs from $[\poly(N)]$, and maximum degree $\Delta$ that are $D$-radius-identical to $B_D(v)$, i.e., the set of possible inputs to $\mathcal{A}_{\LOCAL}$ for which $v$ would see $B_D(v)$ as its $D$-radius ball. For each $G\in \mathcal{H}_v$, $v$ creates a simulation graph $\Gamma_G$ as follows: $\Gamma_G$ consists of $\lfloor \frac{N^{R+2}}{n_G} \rfloor \ge n_G^r$ disjoint copies of $G$. One of these copies is arbitrarily designated the `true' copy, and its nodes use the IDs of $G$ as their own IDs and names. All other copies use the same IDs, but as names they use arbitrary unique values in $[\poly(N)]$. We also add enough isolated nodes to raise the number of nodes to exactly $N^{R+2}$ (i.e., $N^{R+2}-n_G\lfloor \frac{N^{R+2}}{n_G} \rfloor < n_G$ isolated nodes), sharing the same arbitrary ID, and with arbitrary unique names, in $[\poly(N)]$.

We will be running $\mathcal{A}_{\MPC}$ on this simulation graph $\Gamma_G$. For the supply of randomness, denote $\mathcal{S}'$ to be $\mathcal{S}$ curtailed to the length required by $\mathcal{A}_{\MPC}$, i.e., the first $\poly(N)$ bits. Since $\mathcal{A}_{\MPC}$ is component-stable, its output at $v$ on $\Gamma_G$, using seed $\mathcal{S}'$, is $\mathcal{A}_{\MPC}(G,v,N^{R+2},\mathcal{S}')$.

Then, we set

\begin{align*}
    \mathcal{A}_{\LOCAL} (H,v,\mathcal{S}) &:=
    \arg \max_{x} |\{G\in \mathcal{H}_v: \mathcal{A}_{\MPC}(G,v,N^{R+2},\Delta,\mathcal{S}')=x \}|
    \enspace,
\end{align*}
%
i.e., $v$'s output label is that returned by the most $\mathcal{A}_{\MPC}$ simulations.

\paragraph{Correctness of the \LOCAL algorithm.}

By our assumption that $\mathcal{A}_{\MPC}$ is not sensitive, we now have that for any $G, G'\in \mathcal{H}_v$, with probability at least $1-\eps$ over choice of $\mathcal{S}$, $\mathcal{A}_{\MPC}(G,v,N^{R+2},\mathcal{S}')= A_{\MPC}(G',v,N^{R+2},\Delta,\mathcal{S}')$. So, in particular, since the actual input graph $H$ is certainly in $\mathcal{H}_v$,

\begin{align*}
\mathbf E_{\mathcal{S}}\left[ \frac {|\{G\in \mathcal{H}_v:A_{\MPC}(G,v,N^{R+2},\Delta,\mathcal{S}')\ne A_{\MPC}(H,v,N^{R+2},\Delta,\mathcal{S}') \}|}{|\mathcal{H}_v|}\right]\le\eps\enspace.
\end{align*}

Then, for random $\mathcal{S}$, the probability that
\[ \frac {|\{G\in \mathcal{H}_v:A_{\MPC}(G,v,N^{R+2},\Delta,\mathcal{S}')\ne A_{\MPC}(H,v,N^{R+2},\Delta,\mathcal{S}') \}|}{|\mathcal{H}_v|}\ge \frac 12\] is at most $2\eps$ by Markov's inequality. We therefore have \[\Prob{A_{\LOCAL} (H,v,\mathcal{S}) = A_{\MPC}(H,v,N^{R+2},\Delta,\mathcal{S}')}\ge 1-2\eps\enspace.\]

Taking a union bound over all nodes $v \in V(H)$, we have that with probability at least $1-2N\eps$ over $\mathcal{S}$, $\mathcal{A}_{\LOCAL} (H,v,\mathcal{S}) = A_{\MPC}(H,v,N^{R+2},\Delta,\mathcal{S}')$ for all $v$. In this case, the overall output of $\mathcal{A}_{\LOCAL} (H,\mathcal{S})$ is equal to the output of $\mathcal{A}_{\MPC}$ on the true copy of $H$ when run on $\Gamma_H$ with seed $S'$. Since $\Gamma_H\in\mathcal{G}$ (as it is a disjoint union of members of $\mathcal{G}$),   $\mathcal{A}_{\MPC}$ returns a valid output on $\Gamma_H$ with probability $1-1/n_{\Gamma_H} = 1- N^{-(R+2)}$. Note that $\Gamma_H$ is a disjoint union of at least $n_H^{R}$ copies of $H$ and fewer than $n_H$ extra isolated nodes. This satisfies the construction in the definition of $R$-replicability.\footnote{when $n_H \ge 2$; for $n_H=1$ the lemma is trivial since there can be no \LOCAL lower bounds on such graphs.} Since $\mathcal{A}_{\MPC}$ is component-stable, it must return the same output labeling in all copies of $H$ in $\Gamma_H$ (since they share the same topology and IDs), and likewise must return the same output label on all isolated nodes. So, the output labeling given on $\Gamma_H$ is of the form required in the replicability definition, and so $\mathcal{A}_{\MPC}$ returns a valid output on the true copy (and, indeed, on all copies) of $H$ in $\Gamma_H$.

Then, by a union bound, $\mathcal{A}_{\LOCAL}$'s output is correct with probability at least $1-2N\eps - N^{-(R+2)} \ge 1-1/N$, reaching a contradiction to our assumption of a \LOCAL lower bound. This proves the randomized part of the lemma.

To prove the deterministic analogue, we perform exactly the same construction, except that $\mathcal{A}_{\LOCAL}$ does not have the random seed $\mathcal{S}$, and does not pass it to $\mathcal{A}_{\MPC}$. Since our algorithm $\mathcal{A}_{\LOCAL}$ is now deterministic, we have $\mathcal{A}_{\LOCAL}(H,v) = A_{\MPC}(H,v,N^{R+2},\Delta)$ with certainty for all $v$, i.e., $\mathcal{A}_{\LOCAL}$'s output is identical to $\mathcal{A}_{\MPC}$'s output on an $N^{R+2}$-node graph containing $H$ as a connected component. Since $\mathcal{A}_{\MPC}$ is also deterministic, this is a valid output on $H$ with certainty. We have then constructed a deterministic \LOCAL algorithm solving $\mathcal{P}$, contradicting our initial assumption. So, we must instead have that $\mathcal{A}_{\MPC}$ is $(T(N,\Delta), 1,N^{R+2},\Delta)$-sensitive, and therefore, since it is deterministic, $(T(N,\Delta), 1,N^{R+2},\Delta)$-sensitive.
\end{proof}
}

%---------------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Conditional \MPC lower bounds from \LOCAL}
\label{subsec:stconn}

In this section we apply Lemma \ref{lem:sens} to obtain conditional lower bounds for component-stable \MPC algorithms for $O(1)$-replicable graph problems through their hardness in the \LOCAL model. Our main result, \Cref{thm:lb}, can be seen as a revision and correction of the main arguments due to Ghaffari et al. \cite{GKU19} in their Theorem~I.4, applied to low-space component-stable \MPC algorithms for $O(1)$-replicable graph problems and for normal graph families.

Since the complexity of our algorithms depends on two parameters, input size estimate $N$ and maximum degree $\Delta$, we define the type of functions for which we will study lower bounds:

\begin{definition}%[\textbf{Constrained functions}]
\label{def:constrained-functions}
We call a function $T: \nat \times \nat \rightarrow \nat$ \textbf{constrained} if $T(N,\Delta) = O(\log^\gamma N)$ for all $\Delta \le N$ and $\gamma \in (0,1)$, and $T(N^c,\Delta) \le c \cdot T(N,\Delta)$ for any $c\ge 1$.
%\Artur{Peter: I believe earlier we have been indirectly assuming that $T(N,\Delta) \le \log^{\gamma}n$ for some $\gamma < 1$, and with this, we didn't have to reprove \cite[Lemma~IV.1]{GKU19}, which is needed in the proof of \Cref{thm:lb}. I guess, by setting $T(N,\Delta) = o(\frac{\log N}{\log\log N})$, Peter is implying that the proof holds for such $T(N,\Delta)$ as well, but is this the case? In any case, one should comment about it in the proof of \Cref{thm:lb} below. And this modification can also cause some changes in \Cref{thm:instability-provably-helps}.}
%\Peter{I changed it back}
\end{definition}

This is similar to the corresponding requirement $T(N) = O(\log^\gamma N)$ in \cite{GKU19}, but allowing for dependency on $\Delta$. The definition of constrained functions further incorporates a `smoothness' condition, which is also implicitly required by \cite{GKU19} (there, it is used that when $T(N) = O(\log^\gamma N)$, $T(\poly(N)) = O(T(N))$; while this is true for smooth functions, it is not technically true in general).\footnote{As a counterexample, let $T(N)$ be a tower of 2s of height $\log^*N - 3$. Then, $T(N) = O(\log\log N)$, but $\limsup\limits_{N\to \infty}\frac{T(N+1)}{T(N)} = \infty$.}
%
%\footnote{As a counterexample, let $T(N) = {^{\log^*N - 3}2}$, i.e., a tower $2^{2^{\dots^{2}}}$ of height $\log^*N - 3$. Then, $T(N) = O(\log\log N)$, but $\limsup\limits_{N\to \infty}\frac{T(N+1)}{T(N)} = \infty$.}).\Artur{What is in the last footnote? I cannot parse ``$T(N) = {^{\log^*N - 3}2}$''; is a typo?}\Peter{Apparently that's the most standard notation for a tower of exponentials, but if nobody knows it (I didn't) then maybe we should take it out.}

With the notion of constrained functions at hand, we can leverage Lemma \ref{lem:sens} to relate the complexity of \LOCAL algorithms for $R$-replicable graph problems in normal graph families to the connectivity conjecture. In particular, given the conjectured hardness of this problem in the \MPC model, this will imply (see \Cref{thm:lb} for a precise statement) a lower bound of $\Omega(\log T(n,\Delta))$-rounds for any low-space component-stable \MPC algorithm for any $O(1)$-replicable graph problem in normal graph families with no $T(N,\Delta)$-round \LOCAL algorithm.
%(cf. \cite[Theorem~IV.2]{GKU19})

We begin with an auxiliary lemma that relates Lemma \ref{lem:sens} to the complexity of low-space \MPC algorithms for the $D$-diameter $s$-$t$ connectivity problem.\footnote{The \emph{$D$-diameter $s$-$t$ connectivity problem} is formally defined in \cite[Definition~IV.1]{GKU19} as follows: Given two special nodes $s$ and $t$ in the graph, the goal is to determine whether $s$ and $t$ are connected or not, in a way that provides the following guarantee: If $s$ and $t$ are in the same connected component and that component is a path of length at most $D$ with $s$ and $t$ at its two endpoints, then the algorithm should output \YES, with probability $1 - 1/\poly(n)$. If $s$ and $t$ are in different connected components, the algorithm should output \NO, with probability $1 - 1/\poly(n)$. In other cases, the output can be arbitrary.}

\begin{lemma}
\label{lem:stconn}
Let $\mathcal{P}$ be a $O(1)$-replicable graph problem that has a $T(N,\Delta)$-round lower bound in the randomized \LOCAL model with shared randomness, for constrained function $T$, on graphs with input size estimate $N$ and maximum degree $\Delta$, from some normal family $\mathcal{G}$. Suppose that there is a randomized $o(\log T(n,\Delta))$-round low-space component-stable \MPC algorithm $\mathcal{A}_{\MPC}$ for solving $\mathcal{P}$ on legal $n$-node graphs with maximum degree $\Delta$ from $\mathcal{G}$, succeeding with probability at least $1-\frac1n$. Then, there exists a low-space randomized \MPC algorithm $B_{\text{st-conn}}$ with round complexity $o(\log T(n,\Delta))$ for $T(n,\Delta)$-diameter $s$-$t$ connectivity on graphs with $n$ nodes, succeeding with probability at least $1-\frac1n$.
%\Artur{Do we want to use $T(n,\Delta)$ or $T(N,\Delta)$ here? Don't we want to have \emph{``(\dots) on graphs with $n$ nodes \textcolor[rgb]{0.50,0.00,0.00}{and maximum degree $\Delta$}''}?},
%\Peter{We don't need \Delta for s-t-connectivity, since the problem need only be defined for \Delta = 2.}
%
%Let $\mathcal{P}$ be a $O(1)$-replicable graph problem, with a $T(N,\Delta)$-round randomized lower bound (on \LOCAL algorithms succeeding w.h.p.\Artur{More specific?}) on some normal graph family $\mathcal{G}$ and constrained function $T$. Suppose that there is a randomized $o(\log T(n,\Delta))$-round component-stable \MPC algorithm $\mathcal{A}_{\MPC}$ that solves $\mathcal{P}$ on all $n$-node graphs $G \in \mathcal{G}$, with maximum degree $\Delta$, succeeding with high probability. Then, we obtain a randomized \MPC algorithm $B_{\text{st-conn}}$ with round complexity $o(\log T(n,\Delta))$ for $T(n,\Delta)$-diameter $s$-$t$ connectivity\Artur{Define the problem before our use here. (Use \cite[Definition~IV.1]{GKU19}?)} on graphs with $n$ nodes, succeeding with high probability.
	
The same holds if the \LOCAL lower bound and algorithm $\mathcal{A}_{\MPC}$ are both deterministic (but the obtained \MPC algorithm $B_{\text{st-conn}}$ is still randomized).
\end{lemma}

One point of note in the theorem statement is that we do not make any constraint on the maximum degree of the $s$-$t$ connectivity instance; indeed, for that problem any node of degree over $2$ can be immediately discarded, so maximum degree is largely irrelevant. $\Delta$ appears only in the expression for the diameter $D$.

\begin{proof}
Let $c$ be a sufficiently large constant. We will require that $\mathcal{P}$ is $\frac{c}{\sparam}$-replicable; since replicability is monotone, this will be the case when $c$ is sufficiently large. We then construct our randomized \MPC algorithm for $T(n,\Delta)$-diameter $s$-$t$ connectivity $B_{\text{st-conn}}$ as follows:

We are given an $n$-node input graph $H$, and $\poly(n)$-bit random seed $\mathcal{S}$, for $T(n,\Delta)$-diameter $s$-$t$ connectivity. We set $N=n^{\sparam/2}$, denote $D:= T(N,\Delta)$, and apply Lemma \ref{lem:sens} to obtain\footnote{Lemma \ref{lem:sens} shows the \emph{existence} of such graphs, but a uniform \MPC algorithm must also be able to \emph{find} them (a non-uniform algorithm can simply have them `hard-coded' in). To do so, we can run a brute-force search on each machine; $O(n^{\sparam})$ space is required to identify each of the $2^{O(n^{\sparam})}$ pairs of graphs and check the sensitivity property. However, we require $2^{O(n^{\sparam})}$ local computation (which is also implicitly the case in \cite{GKU19}). For specific lower bounds there may be efficient constructions, but this must be determined on a case-by-case basis.} two $D$-radius-identical centered graphs $G,G'\in \mathcal{G}$ with at most $ N$ nodes and maximum degree $\Delta$, such that $\mathcal{A}_{\MPC}$ is $(D, \frac{1}{4N^2},n^{c/\sparam+2},\Delta)$-sensitive with respect to $G,G'$.
		
Our algorithm $B_{\text{st-conn}}$ will work by combining the results of several parallel simulations, run on disjoint groups of machines. We first divide the seed $\mathcal{S}$ equally among these simulations; by choosing our input $\poly(n)$ seed length sufficiently high, we can guarantee that each simulation is given sufficient randomness. In each simulation, each node in $v\in V(H)$ uses part of the random seed assigned to the simulation to independently, uniformly randomly, choose a value $h(v) \in [D]$.

For each simulation we now construct a pair of graphs $G_H$ and $G'_H$ on which to run $\mathcal{A}_{\MPC}$. In each case we begin with the graph $H$, and discard all nodes of degree higher than $2$. Then, for each remaining node in $H$ we collect its radius-$1$ neighborhood onto a machine (this takes $O(1)$ rounds and does not increase asymptotic space usage). Each node of $H$ then drops out if its radius-$1$ neighborhood is not consistent with being part of an $s-t$ path with consecutively increasing values of $h$ along the path (other than the value of $h(t)$, which we make no requirements for). In particular:
		
\begin{itemize}
\item Nodes $s$ and $t$ in $H$ must have degree $1$ (and otherwise we terminate the simulation immediately and output \NO).
\item Other nodes must have degree $2$, and the values of $h$ in their radius-$1$ neighborhood must be a consecutive triplet (other than $h(t)$).
\end{itemize}
		
Now, every remaining node (i.e., satisfying these conditions) in $H$ is assigned (copies of) nodes in $G$ and $G'$ as follows:
		
\begin{itemize}
\item Node $s$ in $H$ is assigned all nodes of distance at most $h(s)$ from $v$ in $G$ and $G'$.
\item Node $t$ in $H$ is assigned all nodes of distance more than $D$ from $v$ in $G$ and $G'$.
\item Other nodes $u$ in $H$ are assigned the nodes of distance exactly $h(u)$ from $v$ in $G$ and $G'$.
\end{itemize}
		
We can now define the new graphs $G_H$ and $G'_H$ as follows:

The node sets of $G_H$ and $G'_H$ consist of every assigned copy of nodes in $G$ and $G'$ respectively. We also add to $G_H$ and $G'_H$ an extra, full, copy of $G$, disconnected from the rest of the graph, whose sole purpose is to ensure that the maximum degree of $G_H$ and $G'_H$ is exactly $\Delta$, and enough isolated nodes to raise the number of nodes (currently $O(nN) = O(n^{1+\sparam/2})$) to exactly $n^{c/\sparam +2}$ (which is larger for sufficiently large constant $c$). Let $w_{u}$ in $G_H$ denote a copy of $w$ in $G$, assigned to node $u$ in $H$. We place an edge between $w_{u}$ and $\hat w_{\hat u}$ in $G_H$ iff $w\sim_G \hat w$ and $u\sim_H \hat u$ (or $u=\hat u$). As IDs, for a simulated node $w_{u}$, we use the original ID of $w$. We will show that these IDs remain component-unique in $G_H$ and $G'_H$. As names, we use $(name(u),name(w))$; these names are guaranteed to be fully unique. We arbitrarily choose fully unique names and IDs for the extra isolated nodes and copy of $G$.


The graphs $G_H$ and $G'_H$ can easily be constructed in $O(1)$ rounds of \MPC, using $O(n^{\sparam})$ local space, since machines each need only store $G$, $G'$, and $O(n^{\sparam})$ edges of $H$. We construct $G'_H$ from $G'$ analogously.
		
We see that the connected components of $G_H$ and $G'_H$ are isomorphic to induced subgraphs of $G$ and $G'$ respectively. Furthermore, the IDs of nodes in these components are identical to the relevant subgraphs of $G$ and $G'$, and are therefore component-unique (as they were in $G$ and $G'$). In particular, we consider the topology and IDs of the connected components $CC({v_{s}})$ and $CC'(v_{s})$ containing $v_{s}$ in $G_H$ and $G'_H$ respectively:
		
\begin{enumerate}
\item If $s$ and $t$ are endpoints of a path of $p\le D+1$ \emph{nodes} (and therefore of \emph{length} at most $D$) in $H$, $h(s)=p-D$, and $h(u_d) = p-D+d$ for each $u_d\ne t$ which is the node at distance $d$ along the path from $s$, then $CC({v_{s}}) =  G$ and $CC'(v_{s}) = G'$;
\item otherwise, $CC(v_{s})=CC'(v_{s})$.
\end{enumerate}
		
In the first case, this is because the nodes on the $s-t$ path are together assigned precisely one copy of each on the nodes in $G$ and $G'$, in such away that every two adjacent nodes in $G$ and $G'$ are assigned to adjacent nodes on this path. In the second case, the only nodes that differ in $G$ and $G'$ are assigned only to $t$, and no outputs of $h$ can cause these to be connected to $v_{s}$. Therefore the graphs of nodes that \emph{are} connected to $v_{s}$ are identical.
	
We now simulate $\mathcal{A}_{\MPC}$ on $G_H$ and $G'_H$ using a sufficiently large $\poly(n)$-length part of $\mathcal{S}$ allocated to this simulation as the random seed (the same seed for both $G_H$ and $G'_H$). Since $G_H$ and $G'_H$ are in the \emph{normal} family $\mathcal{G}$ (they are disjoint unions of induced subgraphs of $G, G'\in \mathcal{G}$), these are valid inputs for $\mathcal{A}_{\MPC}$.
		
If $s$ and $t$ are endpoints of a path of length at most $D$ in $H$, then the probability that all nodes $v$ on this path choose the `correct' value $h(v)$ (i.e., as specified in point $1$ above) is at least $D^{-D} = N^{-o(1)}$. In this case, we have $CC({v_{s}}) =  G\in \mathcal{G}$ and $CC'(v_{s}) = G'\in \mathcal{G}$. Since $\mathcal{A}_{\MPC}$ is component-stable, its output for $v_{s}$ in each case is equal to $\mathcal{A}_{\MPC}(G,v,n^{c/\sparam+2},\Delta,\mathcal{S})$  and $\mathcal{A}_{\MPC}(G',v,n^{c/\sparam+2},\Delta,\mathcal{S})$ respectively, and by sensitivity, with probability at least $\frac{1}{4N^2}$, these are different. If this occurs, the simulation output, and the overall output, is correctly~\YES.

If $s$ and $t$ are not endpoints of a path of length at most $D$ in $H$, then in all simulations we have $CC({v_{s}})=CC'({v_{s}})$. Since $\mathcal{A}_{\MPC}$ is component-stable, its output depends (deterministically) on these connected components (as well as equal values of $\Delta$, random seed $\mathcal{S}$, and $n_{G_H}=n_{G'_H}=n^{c/\sparam+2}$), and is therefore the same in both cases. The output of all simulations is then correctly~\NO.
				
The final output for $B_{\text{st-conn}}$ is as follows: after running $\poly(n)$-many concurrent simulations, we return \YES if any simulation returned \YES, and \NO otherwise. We have already shown that if $s$ and $t$ are not endpoints of a path of length at most $D$ in $H$, all simulations will return \NO, so $B_{\text{st-conn}}$ will correctly output \NO. It remains to show that $B_{\text{st-conn}}$ is also correct with high probability on \YES instances.

Each simulation has a $D^{-D} = N^{-o(1)}$ probability of the nodes in the s-t path choosing the correct values of $h(v)$, and a $\frac{1}{4N^2}$ probability of returning different outputs on $G_H$ and $G'_H$. Therefore, there is at least a $\frac{1}{4N^3}$ probability of the simulation returning \YES. Since simulations use independent randomness, and we can run sufficiently large $\poly(n)$ many of them in parallel, we can amplify the total probability of success to $1-\frac {1}{n}$ as required.

The round complexity of $B_{\text{st-conn}}$ is dominated by simulating $\mathcal{A}_{\MPC}$ on graphs with $O(n^{c/\sparam+2})$ nodes and maximum degree $\Delta$, which, using that $T$ is a constrained function, is $O(T(n^{c/\sparam+2},\Delta)) = O(T(n,\Delta))$.
\end{proof}

%---------------------------------------------------------------------------------------------------------------------------------------------------------

While Lemma \ref{lem:stconn} already provides a strong conditional lower bound for $O(1)$-replicable graph problems in our setting, the lower bound is conditioned on the complexity of solving $D$-diameter $s$-$t$ connectivity. However, we can apply the framework \cite{GKU19} to extend the analysis to condition on the more standard \emph{connectivity conjecture}.

\begin{theorem}
\label{thm:lb}
Let $\mathcal{P}$ be a $O(1)$-replicable graph problem that has a $T(N,\Delta)$-round lower bound in the randomized \LOCAL model with shared randomness, for constrained function $T$, on graphs with input estimate $N$ and maximum degree $\Delta$, from some normal family $\mathcal{G}$. Suppose that there is a randomized $o(\log T(n,\Delta))$-round low-space component-stable \MPC algorithm $\mathcal{A}_{\MPC}$ for solving $\mathcal{P}$ on legal $n$-node graphs with maximum degree $\Delta$ from $\mathcal{G}$, succeeding with probability at least $1-\frac 1n$. Then, there exists a low-space randomized \MPC algorithm $\mathcal{A}_{cycle}$ that can distinguish one $n$-node cycle from two $\frac{n}{2}$-node cycles in $o(\log n)$ rounds, succeeding with probability at least $1-\frac 1n$.
	
The same holds if the \LOCAL lower bound and algorithm $\mathcal{A}_{\MPC}$ are both deterministic (but the obtained algorithm $\mathcal{A}_{cycle}$ remains randomized).
\end{theorem}

\begin{proof}
This reduction is taken directly from Section~V in \cite{GKU19}. First, we notice that \cite[Lemma~IV.1]{GKU19} applies to any \MPC algorithm, i.e., is not affected by our changes to the definition of component-stability. Therefore, assuming that any low-space \MPC algorithms distinguishing one $n$-node cycle from two $\frac{n}{2}$-node cycles requires $\Omega(\log n)$ rounds, we obtain that any low-space \MPC algorithm that solves $D$-diameter $s$-$t$ connectivity for\Artur{As I wrote next to Definition \ref{def:constrained-functions}, now we do not require that $D \le \log^\gamma n$ but only $D = O(\log n/\log\log n)$. One should polish this. (And whatever bound we have here, we use it also in the proof/statement of \Cref{thm:instability-provably-helps}. Now I left it with $T_r(N) < \log^{\gamma} N$ but one should double-check what is with the new Definition \ref{def:constrained-functions})} $D \le \log^\gamma n$ for a constant $\gamma \in (0, 1)$ requires $\Omega(\log D)$ rounds.
%
Now, by setting $D = T(n,\Delta)$, we can combine this fact with Lemma \ref{lem:stconn} to conclude the proof of the theorem.
%that with the assumption of the theorem, the existence of an $o(\log T(N,\Delta))$-round low-space component-stable \MPC algorithm $\mathcal{A}_{\MPC}$ for solving $\mathcal{P}$ on $\mathcal{G}$, succeeding with high probability, yields a low-space randomized \MPC algorithm that can distinguish one $n$-node cycle from two $\frac{n}{2}$-node cycles in $o(\log n)$ rounds, succeeding with high probability.
\end{proof}

\junk{
\subsection{Conditional \MPC lower bounds via hardness of 1-vs-2-cycle conjecture}
\label{subsec:thm:lb}

While Lemma \ref{lem:stconn} already provides a strong conditional lower bound for $O(1)$-replicable graph problems in our setting, the lower bound is conditioned on the complexity of solving $D$-diameter $s$-$t$ connectivity, which has not been studied so extensively in the past. In what follows, we apply the approach from \cite{GKU19} to extend the analysis to condition on the more standard \emph{1-vs-2-cycle conjecture}. We begin with the following lemma (proven by Ghaffari et al.\ \cite{GKU19} in the setting of a different notion of component-stable algorithms, as discussed in \Cref{subsec:problems-with-def-comp-stab}).
%
%We can now apply Lemma IV.1\Artur{Please always refer to a published version of \cite{GKU19}, which is in the FOCS proceedings.} of \cite{GKU19} to reach the more standard 1-vs-2-cycle conjecture as a condition:

\begin{lemma}%[\textbf{\cite[Lemma~IV.1]{GKU19}}]
\label{lem:1v2cycle}
Suppose that every \MPC algorithm with local memory $\spac = n^\sparam$ for a constant $\sparam \in (0,1)$ and global memory $\poly(n)$ that can distinguish one $n$-node cycle from two $\frac{n}{2}$-node cycles requires $\Omega(\log n)$ rounds. Then, any \MPC algorithm with local memory $\spac = n^\sparam$ and global memory $\poly(n)$ that solves $D$-diameter $s$-$t$ connectivity for $D\le \log^\gamma n$ for a constant $\gamma \in (0, 1)$ requires $\Omega(\log D)$ rounds.
\end{lemma}

\begin{proof}
We use Lemma~IV.1 from \cite{GKU19}. Since this lemma does not require that the algorithm
%for the 1-vs-2-cycle problem\Artur{We should make sure that the \emph{1-vs-2-cycle problem} is defined somewhere.}
is component-stable, our definitional changes have no effect and the proof from \cite{GKU19} applies.
\end{proof}

Now we can combine Lemma \ref{lem:stconn} with Lemma \ref{lem:1v2cycle} to obtain the following theorem.

\begin{theorem}
\label{thm:lb}
Let $\mathcal{P}$ be a $O(1)$-replicable graph problem that has a $T(N,\Delta)$-round lower bound in the randomized \LOCAL model with shared randomness, for constrained function $T$, on graphs with input estimate $N$ and maximum degree $\Delta$, from some normal family $\mathcal{G}$. Suppose that there is an $o(\log T(N,\Delta))$-round\Artur{It was $o(\log D)$-rounds before, and so it was a typo I guess.} low-space component-stable \MPC algorithm $\mathcal{A}_{\MPC}$ for solving $\mathcal{P}$ on $\mathcal{G}$, succeeding with high probability\Artur{More specific? (define what is the failure bound)}. Then, there exists a low-space randomized \MPC algorithm that can distinguish one $n$-node cycle from two $\frac{n}{2}$-node cycles in $o(\log n)$ rounds, succeeding with high probability.
	
The same holds if the \LOCAL lower bound and algorithm $\mathcal{A}_{\MPC}$ are both deterministic.
\end{theorem}

\begin{proof}
Setting $D = T(n,\Delta)$, by Lemma \ref{lem:stconn} we can obtain an $o(\log D)$-round low-space \MPC algorithm for solving $D$-diameter $s$-$t$ connectivity, succeeding with high probability. The theorem then follows from Lemma \ref{lem:1v2cycle}.
\end{proof}
}

%---------------------------------------------------------------------------------------------------------------------------------------------------------

\subsection{Applications of Theorem \ref{thm:lb}: conditional \MPC lower bounds}
\label{subsec:lb:applications}

%\Artur{We might want to have some text here, or we can leave it to other places, where we're proving some lower bounds in \Cref{thm:MIS-MM-1}, \Cref{thm:sinkless-cs}, \Cref{thm:ecoloring-1}, \Cref{thm:vcoloring-1} (deterministic) and Lemma \ref{cor: stableMPC-LB} (randomized).}%
Similarly as it has been demonstrated by Ghaffari et al.\ \cite{GKU19}, the lifting arguments in \Cref{thm:lb} when combined with the known lower bounds for \LOCAL algorithms, lead to a host of conditional lower bounds for low-space component-stable \MPC algorithms for many natural graph problems. In particular, we can recover main applications Ghaffari et al.\ \cite{GKU19} (see Theorems~I.1, I.2, and I.3 there):

\begin{theorem}
\label{thm:recovering-GKU}
Assuming the connectivity conjecture (that no low-space randomized \MPC algorithm can distinguish one $n$-node cycle from two $\frac{n}{2}$-node cycles in $o(\log n)$ rounds, with failure probability $\frac1n$), the following lower bounds hold for low-space randomized \MPC algorithms:
%
\begin{itemize}
\item $\Omega(\log\log n)$ rounds for a constant approximation of maximum matching (even on forests), a constant approximation of vertex cover, a maximal independent set;
\item $\Omega(\log\log\log n)$ rounds for $(\Delta+1)$-coloring, unless the deterministic complexity of $(\Delta+1)$-coloring in the \LOCAL model is $o(\log n)$;
\item $\Omega(\log\log\log n)$ rounds for the Lov\'asz Local Lemma problem, or even for the special instance known as sinkless orientation where we should orient the edges of a $d$-regular graph, where $d \ge 4$, such that each node has at least one outgoing edge.
\end{itemize}
\end{theorem}

\begin{proof}
First, we notice that Ghaffari et al.\ \cite{GKU19} proved the following lower bounds for the randomized \LOCAL model with shared randomness:
%
\begin{itemize}
\item $\Omega(\sqrt{\log n/\log\log n})$ rounds for a $\polylog(n)$-approximate solution for the minimum vertex cover, maximum matching, or minimum dominating set problem, and for finding a maximal matching (even on trees) or a maximal independent set (Theorem~V.1 and Corollary~V.2 in \cite{GKU19});
\item $\Omega(\sqrt{\log\log n})$ rounds for $(\Delta+1)$-coloring unless the deterministic complexity of $(\Delta+1)$-coloring in the \LOCAL model is $o(\log n)$ (indirectly in Corollary~V.4 in \cite{GKU19});
\item $\Omega(\log\log n)$ rounds for the Lov\'asz Local Lemma problem, or even for the special instance known as sinkless orientation where we should orient the edges of a $d$-regular graph, where $d \ge 4$, such that each node has at least one outgoing edge \cite[Corollary~V.5]{GKU19}.
\end{itemize}

The proof of \Cref{thm:recovering-GKU} now follows immediately by combining these \LOCAL lower bound to \Cref{thm:lb}, by taking each time $\mathcal{G}$ to be the set of all graphs, and by noticing that all the problems considered are $O(1)$-replicable (see \Cref{subsec:which-are-replicable-problem}, and for example, Lemma \ref{lemma:LCL-replicable} for \LCL{}s and Lemma \ref{lem:approx-matching-replicable} for approximate maximum matching). Only the approximate lower bound for maximal matching in forests and a constant approximation of maximum matching in forests hold by taking $\mathcal{G}$ to be the set of all forests.
\end{proof}

Comparing the results claimed by Ghaffari et al.\ \cite{GKU19} (Theorems~I.1, I.2, and I.3) with those proven in \Cref{thm:recovering-GKU}, there are only two differences: firstly, our lower bound for matching holds only for forests, while \cite{GKU19} claimed it for trees (though we found some arguments in \cite{GKU19} missing\Artur{Peter: does this sentence make sense? Could we comment on it more, or we don't want to?}), and secondly, our result for $(\Delta+1)$-coloring is updated to hold on a weaker conjecture of no $o(\log n)$-rounds deterministic \LOCAL algorithm for $(\Delta+1)$-coloring (since the original result in \cite{GKU19} conditioned on the $2^{o(\sqrt{\log n})}$-deterministic hardness, which was recently disproved in \cite{RG20}).
%
\Artur{\textcolor[rgb]{0.00,0.46,0.29}{Could we incorporate any new interesting \MPC lower bounds here? Anything \textbf{deterministic}? Anything \textbf{depending on $\Delta$}? This would make this section more exciting, and also our framework more interesting. And notice that since deterministic algorithms don't rely on shared randomness, deterministic \LOCAL lower bounds can be just taken from the standard lower bound in this model. Can we show anything interesting and concrete by combining \Cref{thm:recovering-GKU} with \cite{CKP19} (which shows that for every \LCL problem $\mathcal{P}$, the randomized complexity of $\mathcal{P}$ in the \LOCAL model on graphs of size $n$ is at least the deterministic complexity of $\mathcal{P}$ in the \LOCAL model on graphs of size $\sqrt{\log n}$)?}}


==> randcond.tex <==

\subsection{Sensitivity}



\begin{definition}
	[$(N, D, \eps)$-Sensitive \MPC Algorithm]
	
For an integer $r \ge 0$ and some $\eps > 0$, an \MPC
algorithm A for some graph problem is called $(N,D, \eps)$-sensitive w.r.t. two $D$-hop-identical centered
graphs $G = (V, E)$ and $G' = (V', E')$ with centers $v \in V$ and $v'\in V'$, and valid input size estimate $N$, if the following is true:

We consider two runs of A, one on $G$ and one on $G'$. We take the same uniformly random function $id: ID(A) \rightarrow [N^{3}\eps^{-1}]$ and $poly(N)$-bit random seed $\mathcal S$ for both runs. We apply the function $id$ to map each input node's ID to a new ID in $[N^{3}\eps^{-1}]$; i.e., new IDs are uniformly random, nodes with the same ID in $G$ and $G'$ receive the same new ID, but otherwise IDs are independent. We then run one round of Linial's $O(\Delta^2)$-coloring algorithm, to obtain IDs in $[O(\Delta^2 \log \frac{N^3}{\eps})] = [poly(N,\log \eps)]$. Then, if the \MPC algorithm A is run on $G$ and $G'$, with the new IDs and random seed $\mathcal S$, the probability (over choice of $id$ and $\mathcal S$) that the two centers $v$ and $v'$ output different values is at least $\eps$.
\end{definition}

Note that this definition is only useful with $\eps\gtrapprox 2^{-N^\sparam}$, since otherwise node IDs do not fit onto machines, and the length of the seed is insufficient to give such small probabilities.

\begin{lemma}\label{lem:sens}
Let $P$ be a graph problem for which there is no $T(K,\Delta)$-round LOCAL algorithm that solves $P$ on graphs from some family $\mathcal G$, of maximum degree $\Delta$, with valid input size estimate $K$, with probability at least $1-p(K)$.

Then, for every $N$ with $N^{\beta^2\sparam} \le K \le N^{\beta\sparam}$, for any \MPC algorithm that solves $P$ on $\mathcal G$ with probability at least $1-(1-\frac{3}{4K})p(K)$, given valid input estimate $N$, there are two $T(K,\Delta)$-hop-identical centered graphs $G,G'\in \mathcal G$ with between $K^{\beta}$ and $ K$ nodes and maximum degree $\Delta$, such that $A_{MPC}$ is $(N,T(K,\Delta), \frac{p(K)}{4K})$-sensitive with respect to $G,G'$.

\end{lemma}



\begin{proof}
Denote $D=T(K,\Delta)$ and $\eps = \frac{p(K)}{4K}$. Let us assume that there are not two centered graphs $G$ and $G'$ with $K$ nodes and maximum degree $\Delta$ such that the given \MPC algorithm $A_{MPC}$ is $(N,D,\eps)$-sensitive w.r.t. $G$ and $G'$. We use this fact to construct a $D$-round randomized LOCAL algorithm $A_{LOCAL}$ to solve $P$ on graphs with valid size estimate $K$ with probability at least $1 - p$, which is a contradiction to the assumption of the lemma.

The input for $A_{LOCAL}$ will be a graph $H$ with
\begin{itemize}
	\item a valid input size estimate $K$ (i.e., $K^{\beta}\le|V(H)|\le K$),
	\item $\Delta$, the maximum degree of $H$,
	\item an unbounded random seed $\mathcal S$ .
\end{itemize}

We construct $A_{LOCAL}$ as follows: first, $A_{LOCAL}$ divides its random input $\mathcal S$ into two parts, $\mathcal S_1$ and $\mathcal S_2$, as follows:

\begin{itemize}
	\item $\mathcal S_1$ consists of $poly(N)$ bits and is allocated to provide a seed for simulating $A_{MPC}$
	\item $\mathcal S_2$ is used to give a uniformly random function $id:ID(A_{LOCAL}) \rightarrow [N^{3}\eps^{-1}]$, mapping IDs from the ID space of $A_{LOCAL}$ to new uniformly random IDs in $[N^{3}\eps^{-1}]$.
\end{itemize}


We now fix a node $v$ to consider, and describe how we determine $v$'s output under $A_{LOCAL}$, on a particular input $I=(\mathcal S,H)$. Node $v$ first collects its $D$-radius ball $B_D(v)$ in $H$. It then considers the family $\mathcal H_v$ of all graphs with between $K^{\beta}$ and $ K$ nodes, centered at $v$, with IDs from the ID space of $A_{LOCAL}$, that are $D$-hop-identical to $B_D(v)$, i.e. the set of possible inputs to $A_{LOCAL}$ for which $v$ would see $B_D(v)$ as its $D$-radius ball. For each graph $G\in \mathcal H_v$, $v$ simulates $A_{MPC}$ on $G$, with input estimate $N$, $\mathcal S_1$ as the random seed, the value of $\Delta$, and IDs given by applying the function $id$ to the IDs of $G$ and then running one round of Linial's $O(\Delta^2)$-coloring algorithm (as in the sensitivity definition). We then denote $OUT_{\mathcal S, G} (v)$ to be the output given by $A_{MPC}$ for the node $v$.

Then, we set

\[A_{LOCAL} (\mathcal S,H,v) := \arg \max_{x} |\{G\in \mathcal H_v: OUT_{\mathcal S, G} (v)=x \}|\enspace,\]

i.e., $v$'s output label is that returned by the most $A_{MPC}$ simulations.


\paragraph{Correctness of the LOCAL algorithm}
By our assumption that $A_{MPC}$ is not sensitive, we now have that for any $G, G'\in \mathcal H_v$, with probability at least $1-\eps$ over choice of $\mathcal S$, $OUT_{\mathcal S,G}=OUT_{\mathcal S,G'}$. So, in particular, since the actual input graph $H$ is certainly in $\mathcal H_v$,

\[\mathbf E_{\mathcal S}\left[ \frac {|\{G\in \mathcal H_v:OUT_{\mathcal S,G}\ne OUT_{\mathcal S,H} \}|}{|\mathcal H_v|}\right]\le\eps\enspace.\]

Then, for random $\mathcal S$, the probability that
$ \frac {|\{G\in \mathcal H_v:OUT_{\mathcal S,G}\ne OUT_{\mathcal S,H} \}|}{|\mathcal H_v|}\ge \frac 12$ is at most $2\eps$ by Markov's inequality. We therefore have $\Prob{A_{LOCAL} (\mathcal S,H,v) = OUT_{\mathcal S,H}(v)}\ge 1-2\eps$.

Taking a union bound over all vertices $v \in V(H)$, we have that with probability at least $1-2K\eps$ over $\mathcal S$, the overall output of $A_{LOCAL}(H,K,\Delta,\mathcal S)$ is equal to the output of $A_{MPC}(id(H),N,\mathcal S_1)$. We have $N^\ce\le K^{\beta}\le|V(H)|\le K< N$, so $N$ is a valid input size estimate. Furthermore, with probability at least $1-N^{-1}\eps$ all IDs under $id(H)$ are unique, and the final IDs obtained after applying one round of Linial's algorithm are also unique. So, this is a valid input for $A_{MPC}$, and it solves $P$ with probability at least $1-N^{-1}\eps - (1-\frac{3}{4K})p(K)$. Then, by a union bound, $A_{LOCAL}$'s output is correct with probability at least $1-2K\eps-N^{-1}\eps - (1-\frac{3}{4K})p(K)\ge 1-3K\eps - (1-\frac{3}{4K})p(K)=1-p(K)$.
\end{proof}

%---------------------------------------------------------------------------------------------------------------------------------------------------------


%---------------------------------------------------------------------------------------------------------------------------------------------------------

We now define the type of functions, as algorithmic running times dependent on input size estimate $N$ and maximum degree $\Delta$, for which we will be able to show lower bounds:

\begin{definition}
We call a function $T:\nat\times\nat \rightarrow \nat$ \emph{constrained} if, for all $K,\delta,\in \nat$ and $c\ge 1$, $T(K^c,\Delta) \le c^\gamma T(K,\Delta)$ and  $T(K,\Delta^c) \le c^\gamma T(K,\Delta)$ for some constant $\gamma\in (0,\frac 12)$.
\end{definition}

Note that, in particular, a constrained function $T$ must have $T(K,\Delta)=O(\log^\gamma K\cdot \log^\gamma \Delta)$, and so when $\Delta \le K$ (as will be the case for our purposes), $T(K,\Delta)=O(\log^{2\gamma} K)$.

\begin{lemma}
	Let $P$ be a graph problem with a $D:=T(K,\Delta)$-round randomized lower bound on some graph family $\mathcal G$ and constrained function $T$. Suppose that there is an $o(\log D)$-round component-stable \MPC algorithm $A_{MPC}$ that solves $P$ on all graphs $G\in\mathcal G$, with maximum degree $\Delta$ and valid input estimate $K$. Then, we obtain an \MPC algorithm $B_{st-conn}$ with round complexity $o(\log D)$ for $D$-diameter s-t connectivity on graphs with $poly(K)$ nodes.
\end{lemma}

\begin{proof}

We construct our randomized \MPC algorithm for $D$-diameter s-t connectivity $B_{st-conn}$ as follows:

Assume we are given an $n$-node input graph $H$, with input estimate $N$, and $poly(N)$-bit random seed $\mathcal S$, for $D$-diameter s-t connectivity. Note that our connectivity algorithm $B_{st-conn}$ need not be component-stable, so we can use the exact value of $n$, but our success probability must still depend on $N$. We set $K=n^{\beta\sparam}$, and apply \cref{lem:sens} to obtain two $T(K,\Delta)$-hop-identical centered graphs $G,G'\in \mathcal G$ with between $K^{\beta}$ and $ K$ nodes and maximum degree $\Delta$, such that $A_{MPC}$ is $(n,T(K,\Delta), \frac{1}{3K^2})$ sensitive with respect to $G,G'$.
		
Our algorithm $B_{st-conn}$ will work by combining the results of several parallel simulations, run on disjoint groups of machines. We first divide the seed $\mathcal S$ equally among these simulations; by choosing our input $poly(n)$ seed length sufficiently high, we can guarantee that each simulation is given sufficient randomness, since we will see that only $poly(N)$ random bits per simulation is required. In each simulation, each node in $v\in V(H)$ uses part of the random seed assigned to the simulation to independently, uniformly randomly, choose a value $h(v)\in [D]$.

For each simulation we now construct a pair of graphs $G_H$ and $G'_H$ on which to run $A_{MPC}$. In each case we begin with the graph $H$, and discard all nodes of degree higher than $2$. Then, for each remaining node in $H$ we collect its $1$-hop neighborhood onto a machine (this takes $O(1)$ rounds and does not increase asymptotic space usage). Each node of $H$ then drops out if its $1$-hop neighborhood is not consistent with being part of an $s-t$ path with consecutively increasing values of $h$ along the path (other than the value of $h(t)$, which we make no requirements for). In particular:
		
		\begin{itemize}
			\item Nodes $s$ and $t$ in $H$ must have degree $1$ (and otherwise we terminate the simulation immediately and output \NO).
			\item Other nodes must have degree $2$, and the values of $h$ in their $1$-hop neighborhood must be a consecutive triplet (other than $h(t)$).
		\end{itemize}
		
Now, every remaining node (i.e., satisfying these conditions) in $H$ is assigned (copies of) nodes in $G$ and $G'$ as follows:
		
		\begin{itemize}
			\item Node $s$ in $H$ is assigned all nodes of distance at most $h(s)$ from $v$ in $G$ and $G'$.
			\item Node $t$ in $H$ is assigned all nodes of distance more than $D$ from $v$ in $G$ and $G'$.
			\item Other nodes $u$ in $H$ are assigned the nodes of distance exactly $h(u)$ from $v$ in $G$ and $G'$.
		\end{itemize}
		
We can now define the new graphs $G_H$ and $G'_H$ as follows:

The vertex sets of $G_H$ and $G'_H$ consist of every assigned copy of nodes in $G$ and $G'$ respectively. Let $w_{u}$ in $G_H$ denote a copy of $w$ in $G$, assigned to vertex $u$ in $H$. We place an edge between $w_{u}$ and $\hat w_{\hat u}$ in $G_H$ iff $w\sim_G \hat w$ and $u\sim_H \hat u$ (or $u=\hat u$). We also add an extra, full, copy of $G$, or $G'$ respectively, disconnected from the rest of the graph and given arbitrary unique IDs, whose sole purpose is to ensure that the maximum degree of $G_H$ and $G'_H$ is exactly $\Delta$. The graphs $G_H$ and $G'_H$ can easily be constructed in $O(1)$ rounds of \MPC, using $O(n^{\sparam})$ local space, since machines each need only store $G$, $G'$, and $O(n^{\sparam})$ edges of $H$. We construct $G'_H$ from $G'$ analogously. We choose new identifiers for each node by applying a uniformly random function $id: V(G \cup G') \times V(H)\rightarrow [(nK)^4]$. If two distinct nodes choose the same ID, $B_{st-conn}$ can detect this in $O(1)$ rounds, and the output of that simulation is \NO.
		
We state some basic properties of the graphs $G_H$ and $G'_H$:

\begin{itemize}
	\item The number of nodes in $G_H$ and $G'_H$ is at most the number of vertices in $H$ multiplied by the number in $G$ and $G'$, i.e. at most $nK = n^{1+\beta\sparam}$;
	\item The maximum degree in $G_H$ and $G'_H$ is at most $K = n^{\beta\sparam}$, and the number of edges is at most $n^{1+2\beta\sparam}$ (because each node in $H$ contributes at most $|E(G)|$ and $|E(G')|\le n^{2\beta\sparam}$ edges);
	\item Node IDs are unique with probability at least $1- (nK)^{-2}$;
	\item When the same node in $H$ simulates nodes with the same IDs in $G$ and $G'$, the resulting IDs in $G_H$ and $G'_H$ are the same. Otherwise, they are independent.
\end{itemize}	
		
We also see that the connected components of $G_H$ and $G'_H$ are isomorphic to induced subgraphs of $G$ and $G'$ respectively. In particular, we consider the topology of the connected components $CC({v_{s}})$ and $CC'(v_{s})$ containing $v_{s}$ in $G_H$ and $G'_H$ respectively:
		
		\begin{enumerate}
			\item If $s$ and $t$ are endpoints of a path of $p\le D+1$ \emph{nodes} (and therefore of \emph{length} at most $D$) in $H$, $h(s)=p-D$, and $h(u_i) = p-D+i$ for each $u_i\ne t$ which is the node at distance $i$ along the path from $s$, then $CC({v_{s}}) =  G$ and $CC'(v_{s}) = G'$;
			\item otherwise, $CC(v_{s})=CC'(v_{s})$.
		\end{enumerate}
		
		In the first case, this is because the nodes on the $s-t$ path are together assigned precisely one copy of each on the nodes in $G$ and $G'$, in such away that every two adjacent nodes in $G$ and $G'$ are assigned to adjacent nodes on this path. In the second case, the only nodes that differ in $G$ and $G'$ are assigned only to $t$, and no outputs of $h$ can cause these to be connected to $v_{s}$. Therefore the graphs of nodes that \emph{are} connected to $v_{s}$ are identical.
	
		We now simulate $A_{MPC}$ on $G_H$ and $G'_H$, with input estimate $N_{sim}:=nK$, upper bound $\Delta$ on degrees, and using a sufficiently large $poly(n)$-length part of $\mathcal S$ allocated to this simulation as the random seed (the same seed for both $G_H$ and $G'_H$). Since $G_H$ and $G'_H$ have at most $nK$ vertices, $N_{sim}$ is a valid input estimate. So, as long as IDs in $G_H$ and $G'_H$ are unique (which happens with probability at least $1-2(nK)^{-2}$), these are valid inputs for $A_{MPC}$.
		
If $s$ and $t$ are endpoints of a path of length at most $D$ in $H$, then the probability that all nodes $v$ on this path choose the `correct' value $h(v)$ (i.e., as specified in point $1$ above) is at least $D^{-D} = n^{-o(1)}$. In this case, we have $CC({v_{s}}) =  G\in \mathcal G$ and $CC'(v_{s}) = G'\in \mathcal G$. Since $A_{MPC}$ is component-stable, its output for $v_{s}$ in both cases is equal to its output on $v$ in $G$ and $G'$ respectively, and by $(n,T(K,\Delta),\frac{1}{3K^2})$-sensitivity, with probility at least $\frac{1}{3K^2}$, these are different. If this occurs, the simulation output, and the overall output, is correctly \YES.

If $s$ and $t$ are not endpoints of a path of length at most $D$ in $H$, then in all simulations we have $CC({v_{s}})=CC'({v_{s}})$ (other than when IDs are not unique, in which case we detect this and output \NO for the simulation). Since $A_{MPC}$ is component-stable, its output depends (deterministically) on these connected components (as well as equal values of $\Delta$, $N_{sim}$, and random seed), and is therefore the same in both cases. The output of all simulations is then correctly \NO.
				
The final output for $B_{st-conn}$ is as follows: after running $poly(n)$-many concurrent simulations, we return \YES if any simulation returned \YES, and \NO otherwise. We have already shown that if $s$ and $t$ are not endpoints of a path of length at most $D$ in $H$, all simulations will return \NO, so $B_{st-conn}$ will correctly output \NO. It remains to show that $B_{st-conn}$ is also correct with high probability on \YES instances.

Each simulation has a $D^{-D} = n^{o(1)}$ probability of the nodes in the s-t path choosing the correct values of $h(v)$, a $1-(nK)^{-2}$ probability of IDs being unique, and a $\frac{1}{3K^2}$ probability of returning different outputs on $G_H$ and $G'_H$. Therefore, there is at least a $\frac{1}{K}$ probability of the simulation returning \YES. Since simulations use independent randomness, and we can run sufficiently large $poly(n)$ many of them in parallel, we can amplify the total probability of success to at least $1-\frac 1N$, where $N$ is the input estimate of $n$, so long as $N$ is a valid estimate. Then, $B_{st-conn}$ gives the correct output with probability at least $1-\frac 1N$ as required.
	\end{proof}

We can now apply Lemma 4.1 of \cite{GKU19} to reach the more standard 1-vs-2-cycle conjecture as a condition:


\begin{theorem}[Lemma 4.1 of \cite{GKU19}]
Suppose that every \MPC algorithm with local memory $n^\sparam$ for a constant $\sparam \in (0,1)$ and global memory $poly(n)$ that can distinguish one $n$-node cycle from two $n/2$-node cycles requires $\Omega(\log n)$ rounds. Then, any \MPC algorithm with local memory $n^\sparam$ and global memory $poly(n)$ that solves $D$-diameter s-t connectivity for $D\le \log^\gamma n$ for a constant $\gamma \in (0, 1)$ requires $\Omega(\log D)$ rounds.
\end{theorem}

\begin{proof}
Since we do not require that the algorithm for the 1-vs-2-cycle problem is component-stable, our definitional changes have no effect, and the proof from \cite{GKU19} applies.
\end{proof}

\begin{theorem}
	Let $P$ be a graph problem that has a $D = T(N,\Delta)$-round lower bound in the randomized LOCAL model with shared randomness, for constrained function $T$, on graphs with input estimate $N$ and maximum degree $\Delta$ from some family $\mathcal G$. Suppose that there is an $o(\log D)$-round component-stable \MPC algorithm for solving $P$ on $\mathcal G$, with strongly sublinear local memory. Then, there exists a strongly sublinear local memory \MPC algorithm that can distinguish one $n$-node cycle from two $n/2$-node cycles in $o(\log n)$ rounds.
\end{theorem}

\begin{proof}
	content...
\end{proof}
\hide{
{\color{blue}\paragraph{Sketch of PRG for removing $O(\log^* n)$ term}
We compose the non-explicit PRG with the low-space PRG from \cite{NZ96} (but maintaining the property that we can make it explicit by brute-forcing the seed on single machines), to make a new PRG.

The setup is the following: we have a randomized algorithm in which each node takes $n^\eps$ random bits (so we have $poly(n)$ in total, and can write them out as a long seed in which nodes know where to look based on their ID for their own bits). Nodes choose an output label based on these and their balls of radius $r$, which we assume are of size at most $n^\eps$, and we require that with probability at least $\frac 12$, this output label is legal (just for this particular node). We also require that the local computation is $n^O(\eps)$-time, and that the problem is $r$-radius checkable by a LOCAL algorithm (so that a `legal solution' for a node is defined and we can check it for conditional expectations). (I think that latter condition should also be required by your current proof.)

Our random candidate for a PRG is simply a fully random function $\{0,1\}^{O(\eps\log n)}\rightarrow \{0,1\}^{O(n^\eps)}$. I.e., a list of $n^{O(\eps)}$ random $n^{O(\eps)}$-length seeds.

To use the PRG, nodes take each $O(n^\eps)$-length seed given by the function, and give it to the PRG of \cite{NZ96}. In this way they can extend the seed to the $poly(n)$-length seed required for the whole graph and extract their own bits, using $O(n^\eps)$ space in a streaming fashion.

We first look at the number of possible instances our PRG must solve. We have $\binom{poly(n)}{n} = e^{O(n \log n)}$ possible ID assignments on $n$ nodes (with polynomial IDs). Then, for each node, we have an $n^{O(\eps)}$-size circuit, for which there are $e^{n^{O(\eps)}}$ possibilities, so the total amount of inputs to fool is $e^{O(n \log n)}\cdot \left(e^{n^{O(\eps)}}\right)^n = e^{n^{1+O(\eps)}}$.

For any such input, a seed is good if it causes at least $n^{\eps}$ node outputs to be legal. By a bounded-dependence Chernoff-type bound (see e.g. equation 3 of https://arxiv.org/pdf/1811.01404.pdf), a fully random seed would be good for an input with probability at least $1-e^{-n^{1-O(\eps)}}$. The error of the PRG of \cite{NZ96}

Since each seed is independent


We assume that each
}} 
